Implicit Mentoring: The Unacknowledged Developer Efforts in Open Source

Mentoring is traditionally viewed as a dyadic, top-down apprenticeship. This perspective, however, overlooks other forms of informal mentoring taking place in everyday activities in which developers invest time and effort, but remain unacknowledged. Here, we investigate the different flavors of mentoring in Open Source Software (OSS) to define and identify implicit mentoring. We first define implicit mentoring--situations where contributors guide others through instructions and suggestions embedded in everyday (OSS) activities--through formative interviews with OSS contributors, a literature review, and member-checking. Next, through an empirical investigation of Pull Requests (PRs) in 37 Apache Projects, we build a classifier to extract implicit mentoring and characterize it through the dual lenses of experience and gender. Our analysis of 107,895 PRs shows that implicit mentoring occurs (27.41% of all PRs include implicit mentoring) and it does not follow the traditional dyadic, top-down apprenticeship model. When considering the gender of mentor-mentee pairs, we found pervasive homophily--a preference to mentor those who are of the same gender--in 93.81% cases. In the cross-gender mentoring instances, women were more likely to mentor men.

==> OLD_IEEE/conclusion.tex <==
%!TEX root = main.tex

\section{Conclusions and Future Work}


\subsection{Conclusion}
In this paper, we conducted a empirical study for implicit mentoring in OSS.
We replied on data through interviews  with experienced OSS participants to recognize and acknowledge implicit mentoring in OSS.  We conclude that implicit mentoring in OSS is a relationship between developers by giving instructions and suggestions on everyday activities on OSS via multiple channels such as code-review tools, emails, etc. We validated our definition of implicit mentoring through literature review and member-checking survey. 


PR comments on GitHub and similar code-review communication tools are validated that implicit mentoring may potential exist. In addition to this perspective, our machine learning classifier helped us identified 67.53\% out of 974,44 PRs contains implicit mentoring comments, and 70.73\% out of 11,634 developers. Within our findings, we noticed that implicit mentoring is not limited dyadic, top-down approaches, and over-half of implicit mentoring PR-comments are peer-peer mentoring. Our finding may imply that developers are helping with each other despite of seniority.






\boldification{***Having a explicit mentor is not possible for every OSS developer, but the implicit mentoring stay with them for their entire careers in their daily work, and the community would continue pass on the spirit of mutual assistance.}
 
While understand the implicit mentoring, peer mentoring is the majority approaching for implicit mentoring for both GitHub and Project experiences. 
%
%
Recognizing the mentors from from different API may be the motivations to let the OSS community continue pass on the spirit of mutual assistance.
%
In addition, we observed that women are participating mentoring, even women are still minority developers on GitHub. 



\subsection{Future work}

\boldification{***As a future work, we plan to invite more people to interview, therefore, we could cover the activities and definitions as much as possible. }


\boldification{*** In addition, we plan to implement our machine learning as tool to visualize the implicit mentoring for OSS platforms such as GitHub. So that we could encourage more people to be involved in mentoring and help the OSS community move forward quickly.}




==> OLD_IEEE/define.tex <==
\section{Different flavors of mentoring in OSS}
\label{sec:3}

Here, we report on our investigation of different flavors of mentoring in OSS. 

\subsection{Methodology}

We answered our first research question through semi-structured interviews, qualitative analysis, literature survey, and member-checking survey, as shown in Figure~\ref{fig:method} A.

\begin{figure*}[!tbp]
\centering
\includegraphics[width=7in]{pic/method_vertical.png}
\caption{Overview of research method: (A) shows the method used to define implicit mentoring (Section~\ref{sec:3}) (B) presents the method to identify and characterize implicit mentoring (Section~\ref{sec:4}).}
\label{fig:method}
\end{figure*}


\subsubsection{Qualitative analysis on obtained interviews}
We first conducted semi-structured interviews with five OSS developers to learn of their experiences regarding mentoring---both from the perspective of being a mentor and a mentee, when applicable. 
\input{Table/sec3_participant_demo}
\hl{We are not sure if we used snowballing sampling for participants selection}
To do that, we recruited two developers who have spearheaded mentoring programs is OSS and used snowballing sampling method to recruit three additional participants.
The interviews were conducted remotely, lasting around 30 minutes each. 
Each interview was recorded with participants' consent (following university approved IRB protocol) and transcribed. 
Participants were offered a \$50 gift card as compensation for their time.
Table \ref{tab:participant_demo} presents the demographic information of our participants. 



\boldification{At the beginning of the interview, we have explained our goals, and we asked participants about their mentoring experiences including formal and informal}
We briefly explained the goal of the interview to the participants in the beginning of the interview.
We asked participants about their roles and experiences in OSS, their mentoring experiences including formal and informal, and their opinions regarding formal and informal mentoring in OSS. At the end of our interview, we ask participants on how mentoring can be improved in OSS.
We list all our interview questions in the appendix~\cite{}. 



\boldification{We transcribed the interview recordings and we used negotiated agreement to reached a consensus on the code category and rule set}
We transcribed the interview recordings and followed the principles of grounded theory to code for types of mentoring, challenges of mentoring and implicit mentoring. 
Two researchers performed the analysis, by first independently coding all the transcripts via open coding with constant comparison method, during which emerging codes are compared with existing codes. After this step, the two researchers met to discuss their codes and reach negotiated agreement \cite{izquierdo2021long}.


%

\subsubsection{Validating findings from past literature and member checking}
\hl{Anita: what method was done to analyze the papers?}
\boldification{To understand what constitutes mentoring and the different flavors of mentoring research in the field of OSS mentoring, we conduct a narrative literature survey}
To understand what constitutes mentoring and the different flavors of mentoring research in the field of OSS mentoring, we conduct a narrative literature survey~\cite{jahan2016conduct}. \hl{narrative review of the literature}
We focus on the papers from 2012 to 2021 (inclusive) that related to mentoring in top conferences in Software Engineering: IEEE-ICSME, IEEE-RSSE, IEEE-ICGSEW, ACM-FSE, ACM-ESEM, ACM-ICSE, IEEE-ICSME, IEEE-MSR, ACM-SIGCSE, ACM-HCI, and ACM-ICPS. While conducting the literature survey, we searched for a set of keywords from our consensus codesets.


\boldification{In addition to the literature survey, we continue validating our findings through member checking survey.}
We also validated our findings via member checking with our interview participants.
In the member checking phase, we contacted each of our participants through email and sent them a survey which asked if they agreed with our findings. 
Our survey comprised 15 questions, including yes/no, multiple-choice questions, and open-ended questions, if they did not agree with our findings or wanted to add more. 
The survey was conducted via Qualtrics. All our survey questions are attached in the appendix \cite{}. 





\subsection{Results:} 

%Mentoring is important
%there are two types of mentoring, formal, informal
%formal has a lot of chall....
%we found under the informal mentoring, there are two ways explicit/implicit
%the channels of explicit decide it is hard to recognize
%implicit can be recognized and it happens during developers' everyday activities. 
%nobody studied implicit mentoring in OSS, we are the first to define the implicit mentoring

Here, we show the results of our assessment built around mentoring in OSS. 

\subsubsection{Different flavors of mentoring in OSS}
\boldification{Mentoring is much needed, when successful, its awesome, but there are several challenges that exist [...]. Our interviews identified these x challenges ["challenges table" ]}
%
From our qualitative analysis from obtained from interviews, we found two types of mentoring including formal mentoring and informal mentoring. 
Formal mentoring is mentoring programs that held/assigned by organizations such as Google Summer Code \cite{balali2018newcomers, balali2020recommending}.
Informal mentoring is a natural relationship between mentor and mentees based on friendship, through personal and professional experiences \cite{inzer2005review}. However, there are challenges of both kinds of mentoring.


\boldification{Formal mentoring has multiple challenges, especially for formal mentoring}
%
\input{Table/sec3_challenge_table}
As our interview participant P2 mentioned "It's hard to assess during the mentorship."
Overall, out interviews identified seven challenges of mentoring in OSS, as shown in Table~\ref{tab:challenge}. 
A lot of research (Table~\ref{tab:challenge}) as well as organizations have put in work to create formal mentorship programs, but these have specific challenges as our interviewees reported.
The statements are surprising, formal mentoring has lots of challenges, which have been showed by prior studies. 




\boldification{Informal mentoring is more effective than formal mentoring. }
%
Inzer and Crawford \cite{inzer2005review} stated that informal mentoring is more effective than formal mentoring. People regularly go and find informal mentors because of the effectiveness. Unlike formal mentoring, informal mentoring can happens at anytime \cite{ko2018informal}.Our participants stated that "I have always had mentors, all informal mentors, because I chose to learn from them" (P1); "Informal is mostly how I do it all these days" (P5);  "I think informal mentoring, it's something that I really enjoy" (P4), which are inline with these papers \cite{inzer2005review, okurame2005role, ko2018informal}.


\boldification{channels and activities of implicit mentoring indicate that this can be a new direction of investigation}
%
\input{Table/sec3_mentoring_type}
The above quotes from our interviews showed that developers seek out informal mentors explicitly.
However, there is another type of informal mentoring that happens in OSS that is implicit in developers' day to day activities.
For example, P1 said: ``When somebody reviews a patch, that gives a feedback to you, that's a form of mentoring. It’s an informal mentoring". 
And P3 said: ``There's going to be mentors who are more like code reviewers or the design reviewers."
In Figure \ref{tab:mentoring_type}, we show the hierarchical structure of mentoring in OSS, each of the node represents a flavour of mentoring.
Moreover, the channels and activities of implicit mentoring indicate that this can be a new direction of investigation to help the OSS community better understand and recognize informal mentoring, as well as overcome the challenges of formal mentoring.



%while it actually happens a lot [shuah quote], diverging interests (a problem with formal) is not a problem [kate; quote], is important for the project/contribution to be on track [Steve to find quotes], not limited to seniority (P3 "seniority is not important for informal mentoring."), does take time [quote...]

\subsubsection{Definition of implicit mentoring}

\boldification{We define implicit mentoring from three aspects: activities, channels, and frequency.}
%
\input{Table/sec3_valid_table}
We define implicit mentoring from three aspects: activities, channels, and frequency.Implicit mentoring is defined as: ``Mentoring that occurs in OSS developers' \textit{daily} activities, such as \textit{giving suggestions, instructions and addressing errors.}" As for the channels, implicit mentoring may occur over \textit{emails, in-person/remote meetings, and code review tools} such as PR-comments on GitHub. We validated these aspects in our definition in multiple way. Table~\ref{tab:val_tab} presents the different sources of validation for each aspect of implicit mentoring. 



\boldification{We give the conclusion of implicit mentoring}
%
We conclude that implicit mentoring in OSS is a relationship between developers by giving instructions and suggestions on everyday activities on OSS via multiple channels such as code-review tools, emails, etc.


\boldification{However, implicit mentoring is not recognized, we fill the gap by automatically identify implicit mentoring with PR comments.}
%
Unfortunately, implicit mentoring is not well recognized:
P1: ``I believe the employee doesn't have any recognition for [informal] mentorship."
P3: ``No, I don't think the mentorship is recognized at all in the foundation."
In the next section we fill this gap by automatically identifying implicit mentoring within PR comments.

%Story0:
%Mentoring is much needed, when successful, its awesome, but there are several challenges that exist [...]. Our interviews identified these x challenges ["challenges table" ]

%A lot of work in lit as well as regular OSS is put in creating formal mentorship programs, but these have specific challenges our interviews talked about [point to "challenges table"].

%People regularly go and find informal mentors. Although, effortful, many people do that. Quote , which is inline with these papers [paper references].

%...but these have these challenges [ref "challenges table"]

%However, there is another type of informal mentoring that happens in OSS which is implicit in the day to day activities. [Quote]:

%Therefore, mentoring can be seen as these set of activities (figure1: "diff flavors"). 

%here, we explore implicit mentoring deeper, because....while it actually happens a lot [shuah quote], diverging interests (a problem with formal) is not a problem [kate; quote], is important for the project/contribution to be on track [Steve to find quotes], not limited to seniority [], does take time [quote...].

%Implicit mentoring definition:

%Implicit mentoring involves these types of stuff:
%[validation table for Imp. Mentoring definition]

%Implicit mentoring happens in these channels
%[validation table 1 for channels]

%Unfortunately, implicit mentoring is not well recognized: Quote....so, in next section we fill this gap by automatically identifying

%STORY:1

%Formal mentoring has challenges, the satisfaction is missing from both mentor and mentee
%SO....what do I do with this....Why care: not all OSS devs have chance to get formal mentoring...so why try to investigate...how people are getting mentored outside of formal mentoring programs


%Definition/hierarchy of Mentoring- formal/informal (explicit, implicit)


%Informal...explicit is hard to recognize [due to channel == outside of work...]
%SO, why should I care/what do I do

%Channels of implicit mentoring in these communication tools...seems recognizable
%Implicit mentoring definition:giving suggestions/instructions/addressing errors bugs etc.
%So, what do I do with this

%Story2
%There are various mentoring programs for newcomers in OSS. However, they are not very helpful In OSS, developers often get mentored informally. In two ways: Explicitly, by reaching out to people and implicitly, on pull request channels during code reviews and discussions on submitted PRs. Explicit mentoring is hard to identify since they do not happen over public channels. However, implicit mentoring happens very frequently in daily activities on the public communication channels and the developers doing the mentoring go unnoticed and are not acknowledged. We want to understand to what extent implicit mentoring is happening in day-to-day tasks. 


%
%Analysis from qualitative analysis, we observe that the mentoring in OSS has two majority types: formal and informal mentoring. 
%
%As for informal mentoring, Inzer and Crawford state "a relationship between two people where one gains insight, knowledge, wisdom, friendship, and support from the other", which is same in OSS community  \cite{inzer2005review}.
%
%\textbf{However, mentoring is necessary for all developers and organizations, Table indicates that mentoring is happening everyday, it is necessary to find a mentoring system for all developers and organizations.}
%
%However, mentoring is necessary. Software developers needs to learn everyday. P4: "Considering yourself somebody always learning, always, you're always learning more." And the Table \ref{tab:inter} indicate the frequency of the mentoring of each member. 
%
%Thus, it is extremely important to have a appropriate mentoring system for developer in OSS, not just new comers, but for all developers and organizations. 





%\begin{table}[thp]
%\begin{tabular}{|l|l|}
%\hline
%\multicolumn{1}{|c|}{\textbf{Categories}} & \textbf{References} \\ \hline
%"giving instructions"                       & \cite{balali2020recommending}  \cite{steinmacher2012recommending} \cite{fagerholm2014onboarding}                \\ \hline
%"overcoming barriers"                       & \cite{balali2020recommending} \cite{hsieh2013welcome} \cite{fagerholm2014role}                    \\ \hline
%"supporting developments"                   & \cite{hsieh2013welcome} \cite{hsieh2013welcome} \cite{berlin1993beyond} \cite{fagerholm2014role}                    \\ \hline
%"Providing suggestions"                     & \cite{balali2020recommending} \cite{steinmacher2012recommending}                   \\ \hline
%\end{tabular}
%\label{tab:t1}
%\end{table}



















==> OLD_IEEE/discussion.tex <==
%!TEX root = main.tex

\section{Discussion}
%
To the best of our knowledge, we are the first to identify and analyze the implicit mentoring in the OSS community on representative communication platforms, PR-comments.
%
This section discusses the implications of our research and practice from the perspectives.
%
\begin{comment}
@mentor: How to give attribution" @mentor
karma points based on non-coding activity, update profile
Github is changing their profile , we can propose similar
mentoring is big, tip of the iceberg is formal mentorship, this unexplored mentoring keeping the iceberg afloat is yet to be explored
fW: people do topical mentoring...on an avg. x \% of mentoring that happens topical...people who gave one mentpring in a thread...and not paarticipate. We saw that large amt of such act. Further investigate: In a  thread...a comment by an ind...after which other comments happened, but this ind. didnt appear later on. Drive by mentoring..can be good (less effort) but bad (less engagement
\end{comment}





\subsection{Acknowledging implicit mentoring is necessary}
%
\boldification{mentoring is not a one way in OSS, we observed a hierarchical structure of mentoring.}
%
Mentoring system is well-known to help OSS developers mature and enhance completion of projects \cite{balali2018newcomers}. 
Findings from Section \ref{sec:3}, implicit mentoring has not been recognized and acknowledged. However, implicit mentoring happens in OSS developers' daily activities frequently. Recognizing implicit mentoring build a deeply understanding of current status quo of entire mentoring system in OSS. 
In particular, it would be interesting to understand the motivations influencing implicit mentors, and how do the motivations impact the OSS community. P2 stated "...why would I help them unless they are actually going to help me achieve my own personal my own business goals?" Therefore,  our work reminds OSS community the importance of implicit mentoring and how the community is learning from one another and passing on the knowledge other than conventional mentoring system.

\subsection{easy peasy}
Mentoring is seen as a long, formal relationship...but implicit can be can short effort, topical to the PR at hand....in fact, it can even be 1-off (38\%) cases...FILL UP

\subsection{Recognizing implicit mentoring is demand}
Non-coding contributors have been identified in OSS \cite{trinkenreich2020hidden}. As our study proved that contribution to the OSS community also includes efforts not limited to recognized technical activities. Implicit mentoring plays a significant role in OSS, recognizing these activities are demanded to promote the growth of the entire OSS community. Thus, a rewarding system for implicit mentoring in channels like code-review tools would boost the mentoring activities in OSS. 




\subsection{Peer mentoring is the majority approach of implicit mentoring in OSS}
%
\boldification{***On looking deeper in who are the participants, we found that the majority of the mentors are peers of the mentees, peer to peer mentoring is XXX\% of total PR-comments, and peer to peer mentoring is XXX\% for each mentor. }
%
On looking deeper into who are the mentors and mentoring approach, peer mentoring is the majority mentoring approach of implicit mentoring. P4 states that "... seniority is not necessary for implicit mentoring." These findings surprised us and remind us to keep investigating peer mentoring. 
Traditional formal mentoring is the top to down approaching, but it is studied to indicate that formal mentoring programs are designed for newcomers \cite{fagerholm2014role,balali2018newcomers, balali2020recommending}. Our findings indicate that developers bring their experiences outsides of OSS and contribute to the OSS community, and help each other by sharing knowledge, giving suggestions/instructions, and identifying errors. The online communities can also leverage the classifier to identify and acknowledge implicit mentoring




\subsection{Women OSS developers are not just contributors in OSS but mentors}

\boldification{***We found that there are more men than women are doing implicit mentoring, but we also know that women are under-represented in OSS which might affect these numbers. In addition, our findings indicate that even women are minority in OSS, but they are participating contribution and mentoring.}

Based on the gender dimensions, we found that there are more men than women are doing implicit mentoring, but we also know that women are under-represented in OSS which might affect these numbers.
%
Finding from our gender distribution, we noticed even women are minority in OSS, but they are still participating mentoring.
%
In addition, multiple studies state that cross gender mentoring is effective.
%
Our finding would motivate gender diversity in implicit mentoring in OSS.


==> OLD_IEEE/extra.tex <==
\subsection{Mentoring in OSS}

To get an overview of the current state-of-the-art research in the field of OSS  mentoring, we conduct a literature survey. We focus on the papers from 2012 to 2021 (inclusive) that related to mentorship in top conferences in Software Engineering: IEEE-ICSME, IEEE-RSSE, IEEE-ICGSEW, ACM-FSE, ACM-ESEM, ACM-ICSE, IEEE-ICSME, IEEE-MSR, ACM-SIGCSE, ACM-HCI, and ACM-ICPS.

While conducting the literature survey, we searched for a set of keywords including mentoring in OSS, mentorship in OSS, implicit mentoring in OSS, informal mentoring software engineer etc. We found 23 papers on mentoring in OSS. And Table \ref{tab:literaturesurvey} presents the summary of the literature survey for most recent 10 years. 

\zf{Table may move to appendix later}
\begin{table}[t]
\label{tab:literaturesurvey}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll|l|l|}
\cline{3-4}
                                                                        &                                                                                                                         & \cellcolor[HTML]{FCFF2F}{\color[HTML]{000000} } & Explicit mentoring for newcomers  \\ \cline{3-4} 
                                                                        &                                                                                                                         & \cellcolor[HTML]{FFCE93}                        & Explicit mentoring programs       \\ \cline{3-4} 
                                                                        &                                                                                                                         & \cellcolor[HTML]{9AFF99}                        & Potential implicit mentoring      \\ \hline
\multicolumn{1}{|l|}{\textbf{Index}}                                    & \textbf{Title}                                                                                                          & \textbf{Year}                                   & \textbf{Conference}               \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}1}                         & Recommending Tasks to Newcomers in OSS Projects: How Do   Mentors Handle It?                                            & 2020                                            & ACM-ICPS                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}2}                         & Training the future workforce through task curation in an OSS   ecosystem                                               & 2016                                            & ACM-FSE                           \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}3}                         & Let Me In: Guidelines for the Successful Onboarding of   Newcomers to Open Source Projects                              & 2019                                            & IEEE-journal                      \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}4}                         & Overcoming open source project entry barriers with a portal   for newcomers                                             & 2016                                            & ACM-ICSE                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}5}                         & X marks the task: Helping developers navigate to the right   task                                                       & 2016                                            & IEEE-HCC                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}6}                         & Determining Newcomers Barrier in Software Development: An IT   Industry Based Investigation                             & 2018                                            & ACM-CSCW                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}7}                         & A Simple NLP-Based Approach to Support Onboarding and   Retention in Open Source Communities                            & 2018                                            & IEEE-ICSME                        \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}8}                         & The role of mentoring and project characteristics for   onboarding in open source software projects                     & 2014                                            & ACM-ESEM                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}9}                         & Onboarding in Open Source Software Projects: A Preliminary   Analysis                                                   & 2013                                            & IEEE-ICGSEW                       \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}10}                        & Supporting newcomers in software development projects                                                                   & 2015                                            & IEEE-ICSME                        \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}11}                        & Recommending mentors to software project newcomers                                                                      & 2012                                            & IEEE-RSSE                         \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}12}                        & Onboarding in Open Source Projects                                                                                      & 2014                                            & IEEE-journal                      \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}13}                        & The hard life of open source software project newcomers                                                                 & 2014                                            & ACM-ICSE                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}14}                        & Do Onboarding Programs Work?                                                                                            & 2015                                            & IEEE-MSR                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}15}                        & Who is going to mentor newcomers in open source   projects?                                                             & 2012                                            & ACM-FSE                           \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}16}                        & Communication strategies for mentoring in software development   projects                                               & 2014                                            & ACM-ICSE                          \\ \hline
\rowcolor[HTML]{FFCE93} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFCE93}{\color[HTML]{000000} 17}} & {\color[HTML]{000000} A theory of the engagement in open source projects via summer   of code programs}                 & {\color[HTML]{000000} 2020}                     & {\color[HTML]{000000} ACM-FSE}    \\ \hline
\rowcolor[HTML]{FFCE93} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFCE93}{\color[HTML]{000000} 18}} & {\color[HTML]{000000} How Long and How Much: What to Expect from Summer of Code   Participants?}                        & {\color[HTML]{000000} 2017}                     & {\color[HTML]{000000} IEEE-ICSME} \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 19}} & {\color[HTML]{000000} Hackathons as an Informal Learning Platform}                                                      & {\color[HTML]{000000} 2016}                     & {\color[HTML]{000000} ACM-SIGCSE} \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 20}} & {\color[HTML]{000000} Informal Mentoring of Adolescents about Computing: Relationships, Roles,   Qualities, and Impact} & {\color[HTML]{000000} 2018}                     & {\color[HTML]{000000} ACM-SIGCSE} \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 21}} & {\color[HTML]{000000} GitHub-OSS Fixit: Fixing Bugs at Scale in a Software   Engineering Course}                        & {\color[HTML]{000000} 2021}                     & {\color[HTML]{000000} ACM-ICSE}   \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 22}} & {\color[HTML]{000000} Why is collaboration needed in OSS projects? a case   study of eclipse project}                   & {\color[HTML]{000000} 2013}                     & {\color[HTML]{000000} ACM-FSE}    \\ \hline
\end{tabular}}
\end{table}


\textbf{***Among the state of art we surveyed from top conference in software engineering, only 2 papers address the implicit mentoring plainly and intentionally, and only focus on teenager computing new learners.}
%
Among the state of art we surveyed, that 16 out 22 studies discussed that mentoring for newcomers, and 2 papers addressed official mentoring programs such as summer of code programs \cite{silva2020theory,silva2017long}, and these program still intend to on-board newcomers. We surprised noticed that only 2 papers address the implicit mentoring plainly and intentionally, but limited for certain group of people in  the field of software engineering. 



\subsection{Implicit mentoring in OSS}



\textbf{***Some literature stated that mentoring happens in GitHub when mentors reviews code. Therefore, we noticed that Pull-request and the comments along with may be a channel that implicit mentoring exist, for example, bug-fix, giving suggestions and instructions.}
%
Tan et. al \cite{tan2021github} find that the GitHub, as one of the most popular OSS community, ensure the code quality by using mentors to review codes. And these activities are not limited to explicit mentoring.  
Hayashi et.al \cite{hayashi2013collaboration} address that singly developer in OSS always only has narrow knowledge, collaborations is one of the methods to over difficulties. For example,  if one committer does not have sufficient knowledge of related parts, collaborations must be taken place to verify and commit the bug-fix. This process can be identified as implicit mentoring, since the collaboration can happens randomly, but the the process including addressing issues, giving instructions, etc. 


\textbf{Mentoring has its own set of challenges, one of which is lack of visibility. This lack of visibility can amount to mentors lose their engineering voice. Some research has shown that this is particularly true for women}
%




\zf{Table may move to appendix later}
\begin{table}[t]
\label{tab:literaturesurvey}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll|l|l|}
\cline{3-4}
                                                                        &                                                                                                                         & \cellcolor[HTML]{FCFF2F}{\color[HTML]{000000} } & Explicit mentoring for newcomers  \\ \cline{3-4} 
                                                                        &                                                                                                                         & \cellcolor[HTML]{FFCE93}                        & Explicit mentoring programs       \\ \cline{3-4} 
                                                                        &                                                                                                                         & \cellcolor[HTML]{9AFF99}                        & Potential implicit mentoring      \\ \hline
\multicolumn{1}{|l|}{\textbf{Index}}                                    & \textbf{Title}                                                                                                          & \textbf{Year}                                   & \textbf{Conference}               \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}1}                         & Recommending Tasks to Newcomers in OSS Projects: How Do   Mentors Handle It?                                            & 2020                                            & ACM-ICPS                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}2}                         & Training the future workforce through task curation in an OSS   ecosystem                                               & 2016                                            & ACM-FSE                           \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}3}                         & Let Me In: Guidelines for the Successful Onboarding of   Newcomers to Open Source Projects                              & 2019                                            & IEEE-journal                      \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}4}                         & Overcoming open source project entry barriers with a portal   for newcomers                                             & 2016                                            & ACM-ICSE                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}5}                         & X marks the task: Helping developers navigate to the right   task                                                       & 2016                                            & IEEE-HCC                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}6}                         & Determining Newcomers Barrier in Software Development: An IT   Industry Based Investigation                             & 2018                                            & ACM-CSCW                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}7}                         & A Simple NLP-Based Approach to Support Onboarding and   Retention in Open Source Communities                            & 2018                                            & IEEE-ICSME                        \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}8}                         & The role of mentoring and project characteristics for   onboarding in open source software projects                     & 2014                                            & ACM-ESEM                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}9}                         & Onboarding in Open Source Software Projects: A Preliminary   Analysis                                                   & 2013                                            & IEEE-ICGSEW                       \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}10}                        & Supporting newcomers in software development projects                                                                   & 2015                                            & IEEE-ICSME                        \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}11}                        & Recommending mentors to software project newcomers                                                                      & 2012                                            & IEEE-RSSE                         \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}12}                        & Onboarding in Open Source Projects                                                                                      & 2014                                            & IEEE-journal                      \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}13}                        & The hard life of open source software project newcomers                                                                 & 2014                                            & ACM-ICSE                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}14}                        & Do Onboarding Programs Work?                                                                                            & 2015                                            & IEEE-MSR                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}15}                        & Who is going to mentor newcomers in open source   projects?                                                             & 2012                                            & ACM-FSE                           \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}16}                        & Communication strategies for mentoring in software development   projects                                               & 2014                                            & ACM-ICSE                          \\ \hline
\rowcolor[HTML]{FFCE93} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFCE93}{\color[HTML]{000000} 17}} & {\color[HTML]{000000} A theory of the engagement in open source projects via summer   of code programs}                 & {\color[HTML]{000000} 2020}                     & {\color[HTML]{000000} ACM-FSE}    \\ \hline
\rowcolor[HTML]{FFCE93} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFCE93}{\color[HTML]{000000} 18}} & {\color[HTML]{000000} How Long and How Much: What to Expect from Summer of Code   Participants?}                        & {\color[HTML]{000000} 2017}                     & {\color[HTML]{000000} IEEE-ICSME} \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 19}} & {\color[HTML]{000000} Hackathons as an Informal Learning Platform}                                                      & {\color[HTML]{000000} 2016}                     & {\color[HTML]{000000} ACM-SIGCSE} \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 20}} & {\color[HTML]{000000} Informal Mentoring of Adolescents about Computing: Relationships, Roles,   Qualities, and Impact} & {\color[HTML]{000000} 2018}                     & {\color[HTML]{000000} ACM-SIGCSE} \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 21}} & {\color[HTML]{000000} GitHub-OSS Fixit: Fixing Bugs at Scale in a Software   Engineering Course}                        & {\color[HTML]{000000} 2021}                     & {\color[HTML]{000000} ACM-ICSE}   \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 22}} & {\color[HTML]{000000} Why is collaboration needed in OSS projects? a case   study of eclipse project}                   & {\color[HTML]{000000} 2013}                     & {\color[HTML]{000000} ACM-FSE}    \\ \hline
\end{tabular}}
\end{table}


Among these papers, most of the papers focus on the importance, challenges, and benefits of the mentoring. We analyze the amount and kinds of the mentoring they investigated. We notice that 14 studies discussed that mentoring for newcomers, and 2 papers discussed the benefits from mentoring programs such as summer of code programs \cite{silva2020theory,silva2017long}, these program still intend to on-board newcomers. We surprised noticed that only 2 papers address the implicit mentoring plainly and intentionally. 


\begin{table}[htb]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll}
\hline
\textbf{Repository}            & \textbf{Language}                     \\ \hline
\rowcolor[HTML]{EFEFEF} 
{\color[HTML]{000000} Archiva} & {\color[HTML]{000000} Java}           \\
Aries                          & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
{\color[HTML]{000000} Beam}    & {\color[HTML]{343434} Java/Python}    \\
Cassandra                      & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Cloudstack                     & Java/Python                           \\
CXF                            & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Geronimo                       & Java                                  \\
Groovy                         & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Hbase                          & Java                                  \\
Hive                           & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Ignite                         & Java/C\#/C++/SQL/JDBC/ODBC            \\
Isis                           & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Jackrabbit                     & Java                                  \\
Jclouds                        & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Jena                           & Java                                  \\
Karaf                          & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Log4j                          & Java                                  \\
Maven                          & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Mesos                          & C++                                   \\
OFBiz                          & Java/Groovy/JavaScript/XML/Freemarker \\
\rowcolor[HTML]{EFEFEF} 
Phoenix                        & Java/SQL                              \\
Qpid                           & Java/C\#/C++/Perl/Python/Ruby         \\
\rowcolor[HTML]{EFEFEF} 
Storm                          & Java                                  \\
Subversion                     & C\#                                   \\
\rowcolor[HTML]{EFEFEF} 
TomEE                          & Java                                  \\
Wicket                         & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Ant                            & Java                                  \\
Camel                          & Java/CML                              \\
\rowcolor[HTML]{EFEFEF} 
FOP                            & Java                                  \\
JMeter                         & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
POI                            & Java                                  \\
Tinkerpop                      & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Tomcat                         & Java                                  \\
Usergrid                       & Java/JavaScript/PHP/HTML              \\
\rowcolor[HTML]{EFEFEF} 
Hadoop                         & Java                                  \\
Spark                          & Java/Scala/Python/R/SQL/JDBC          \\
\rowcolor[HTML]{EFEFEF} 
Flink                          & Java/Scala                           
\end{tabular}}
\label{tab:apacheprojects}
\end{table}




\begin{table}[tbp]
\centering
\begin{tabular}{lll}
\multicolumn{3}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Top to down}}    \\ \hline
                     & \textbf{Total}      & \textbf{Mentoring}     \\
Male                 & 114,982             & 38,718                 \\
Female               & 1,103               & 486                    \\
\multicolumn{3}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Bottom up}}      \\ \hline
                     & \textbf{Total}      & \textbf{Mentoring}     \\
\textbf{Male}        & 326,59              & 11,133                 \\
\textbf{Female}      & 638                 & 262                    \\
\multicolumn{3}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Peer mentoring}} \\ \hline
                     & \textbf{Total}      & \textbf{Mentoring}     \\
\textbf{Male}        & 164,993             & 58,620                 \\
\textbf{Female}      & 6,549               & 1,995                 
\end{tabular}
\label{tb:gender_pro_count}
\end{table}


==> OLD_IEEE/identify.tex <==
\section{Implicit mentoring and its characteristics}


\label{sec:4}

\boldification{we answer RQ2 by focusing on PR comments because...}
In this section, we report on how to identify and characterize implicit mentoring in OSS projects (RQ \#2). Our goal here is to investigate how to automate the identification of implicit mentoring taking place on an everyday basis, but remaining unacknowledged.
Here we focus on implicit mentoring occurring via PR-comments as it a prominent channel via which developers provide feedback and mentoring as found by Kononenko et al.~\cite{kononenko2018studying} and mentioned by our interview participants (cf. Section~\ref{sec:3}). 


\boldification{past work shows mentoring to be dyadic, topc-down, we investigate this}
Traditionally, mentoring has been viewed as a dyadic relationship wherein an experienced individual (the mentor) provides practical advice and guidance to an inexperienced individual (the mentee)~\cite{Kram_1988, gandhi2012reverse}, helping them gain technical and job-related skills~\cite{brashear2006exploratory, hale2000match}. Therefore, we wanted to analyze if the same sort of mentoring dynamics occur in implicit mentoring, leading to:\\
\textit{RQ2a: To what extent is implicit mentoring characterized by dyadic, top-down interactions?}. 


\boldification{past work has shown women do more mentoring, low gender numbers, and homophily, so we investigate this}
Additionally, past work has found that women, especially in open source, are more tuned to community building roles~\cite{??} and end up being mentors more often~\cite{??}. This often translates to women seen as community managers and losing their ``engineer" voice in decision making~\cite{??}. Further, given the gender imbalance in OSS (past work having found women contributors to range around 10\% ~\cite{}) and past research having shown that same-gender mentor-mentee dyadic relationships are more common~\cite{}, it can mean that fewer women have mentors. Both of these phenomena disadvantage women in OSS. Therefore, we wanted to investigate if they also occur in implicit mentoring, leading to:\\
\textit{RQ2b: What role do women play in implicit mentoring?}


\subsection{Method}


\boldification{we chose Apache and these projects because...}
Figure \ref{fig:method} B presents the overview of our methods.
\textit{\textbf{Project Selection}}: We use a set of 37 Apache projects as our data corpus to answer RQ\#2. We selected Apache projects since one of the most mature OSS ecosystems with well defined policies and a philosophy of transparency where all discussions should be conducted in online forums, which is essential for us as we aim to extract implicit mentoring from archived communication. Further, the Apache Source Foundation is committed to facilitating and improving mentoring in OSS. In addition to providing explicit guidelines for mentors~\cite{???}, it also oversees one of the most popular formal mentorship programs (The the Google Summer of Code~\cite{??}), which would mean that the philosophy of mentoring is instilled in Apache contributors.  Finally, Apache projects are often studied in scientific research, which allows our work to be placed in the context of existing research~\cite{gharehyazie2015developer,kabinna2016logging,chen2017characterizing,chelkowski2016inequalities,oliva2015evolving}. In fact, we reuse the dataset curated by Mannan et al.~\cite{mannan2020relationship}


\boldification{Our dataset contained this 97,444 PRs and this 588,094 PR comments across these 11,634 authors.}
Table \ref{tab:apache} presents the statistics of the 37 projects in our dataset. The criteria for selecting the dataset was that projects are mature and include sizeable codebase and contributors (which are satisfied by the Mannan et al. dataset). In total, our dataset comprises 97,444 pull-requests, 588,094 PR-comments logged by 11,634 (unique) PR-comment authors. See Supplemental~\cite{Link} for further details about each project in the dataset.
\input{Table/sec4_project_stats}


\boldification{we manually classified implicit mentoring this way and did IRR}
\textit{\textbf{Manual Classification of Sample Data}}: 
To answer our research questions, we need to first differentiate between PR-comments with/without implicit mentoring. As manual classification is not a practical option to classify $588,094$ PR-comments, we use machine learning techniques. To train the machine learning algorithm we needed to manually classify a training set.  
We determine the size of the training dataset by using a 95\% confidence interval and a margin of error of 5\% \cite{kotrlik2001organizational} on the dataset, giving us a sample size of 384 PR-comments.
We then randomly selected the 384 PR-comments from the full dataset to manually classify all its associated comments.


Next, the first two authors manually labeled a subset of the PR-comments in the training set with binary labels based on whether the PR-comment included implicit mentoring to calculate Inter Rater Reliability (IRR) \cite{hallgren2012computing}. A PR-comment was considered to contain implicit mentoring, if it included an ``explanation" in addition to giving suggestions, instructions or helping avoid problems (Table~\ref{tab:rulebook}). 
\input{Table/sec4_rulebook}


The two authors independently labeled 20\% of the PR-comments independently and reached high IRR (94\% Cohen Kappa~\cite{\cite{viera2005understanding}}).The remaining 80\% of the training dataset was split evenly between the two authors who manually classified the PR-comments. 
%


\textit{\textbf{Machine Learning Classifier}}:

Using the manually classified corpus, we train four different machine learning classifiers, aRandom Forest \cite{pal2005random}, a Bernoulli \cite{singh2019comparison}, a Support Vector \cite{cortes1995support}, a KNeighbors \cite{laaksonen1996classification}, and a Decision trees \cite{kothari2001decision}. 

\boldification{Table presents the machine learning classifier comparison results. After comparison, we chose the random forest classifier.}
\input{Table/sec4_ml_results}
%\as{we need to give more details about hyper-parameter optimization}
%\zf{methods are shown in comments}
Table~\ref{tab:ml} shows the precision, recall, F1, and AUC scores of all the classifiers we implemented. 
We used RFC because it had the best overall performance among the five classifiers we implemented. SVM and RFC had similar AUC scores. However, identifying some false positives as mentoring is better than having more false negatives, since we want to minimize undiscovered implicit mentoring instances. Before we select the best performance classifier. To ensure the best performance, we applied hyper-parameter adjustments \cite{horvath2016effects} from Python Scikit learn library \cite{pedregosa2011scikit} to all five classifiers. Randomized look sets up a lattice of hyper-parameter values and chooses arbitrary combinations to train each classifier. By applying $Scikit-Learn RandomizedSearchCV$, we found the optimal parameter for each classifier.Our hyper-parameter grid for the best classifier (Random forester) includes $n_estimators$, $max_features$, $max_depth$, $min_samples_split$, $min_samples_leaf$, and $bootstrap$. The final tuned Random forester parameters for our classifier were $n_estimators = 600$, $max_features = auto$, $max_depth = 90$, $min_samples_split = 5$, $min_samples_leaf = 2$, and $bootstrap = True$.  The model was trained with 80\% data sample and tested with 20\% data sample. Thus, we chose the classifier with a greater recall, that is, RFC.
%AYDA TEXT: We performed hyper-parameter optimization using randomized search~\cite{bergstra2012random} for all four classifiers before selecting the decision tree. Randomized search sets up a grid of hyper-parameter values and selects random combinations to train the model and score on the validation data. The number of search iterations is set based on time/resources; in our case, it was 10. We search for the optimal parameter settings using the Scikit-Learn RandomizedSearchCV function. Our hyper-parameter grid for the best classifier (Decision Tree) includes ``max\_depth'',``max\_features'', ``min\_samples leaf'' and ``criterion''. The final tuned decision tree parameters for our classifier were ``min\_samples\_leaf: 5, max\_depth:3, max\_features: 5, criterion: gini''.


\boldification{We need to identify mentors/mentee and their seniority  to answer RQ2a. We identify mentee/mentors this way}
\textit{\textbf{Identifying Expertise of Mentors and Mentees}}: 
In order to investigate the extent to which top-down interactions comprise implicit mentoring (RQ2a), we need to first identify when someone is a mentee or a mentor and their experiences. We considered the PR author as a mentee if any of the PR comments associated with that PR is classifed as ``mentoring". Note that, PRs that received no PR comments and were directly accepted or rejected are not included in this analysis. For those PR-comments that are identified as mentoring, their authors are identified as a mentor.


\boldification{we use project/GH exp as a proxy for seniority. We calculate experience this way} 
To investigate the dynamics of implicit mentoring, especially if it comprises top-down interactions (experienced to inexperienced) we calculate experience at two levels. First, experience within the specific project, which we calculated based on the date of their first commit in that project by doing this \as{add me}. However, in OSS, contributors can participate in multiple projects or can leave a project to join another. In such cases, they may bring experiences in working on another project when mentoring a developer in a project. Therefore, we also calculate the overall experience of a mentor in GitHub based on the first commit \as{this way...add me}. Note, that when analyzing the experience of mentors in GitHub, there were cases where the developers had set their profile settings to "private" or had deleted their accounts. There were 413 such profiles (3.43\% of PR-comment authors). To enable a systematic investigation of project-specific and overall experiences, we removed these developers from this analysis in RQ2a.  


\textit{\textbf{Identifying Gender}}: 
\boldification{To investigate the gender diversity of implicit mentoring in OSS, we first mined the information of each mentor we have identified. We applied ``Namsor'' tool to identify the mentor's gender based on the geographic information.}
We also explored the gender dimension of participants to answer RQ2. We know that women are a minority in OSS community \cite{canedo2020work}. Previous research found that mentor relationships involving homogenous or diverse relationships involving female mentors provide more role demonstrations and less professional development than relationships involving male mentors. Homophily man mentoring relationships provided less psychosocial support than woman homophily women relationship \cite{sosik2000role}. Therefore, investigating the gender diversity of OSS implicit mentoring would help the OSS community to understand the effectiveness of mentoring relationship regarding genders. We used the ``Namsor" API to identify their gender based on their full name and geographic information we retrieved from GitHub API. ``NamSor" is a name recognition API that estimates the gender of a name on a -1 to +1 probability scale based on geographic information. \cite{namsor}. Multiple studies have addressed the reliability of the ``Namsor" gender classifications, the error is less than 10\%\cite{santamaria2018comparison, santamaria2018comparison}. Note that not all users had provided their full names and geographic location on GitHub. Thus, after applying the ``Namsor" API, we used the results to do further analysis only if the identified gender probability is over 90\%.


\boldification{we used statistical tests to analyze the gender dimension for implicit mentoring from three aspects: proportions, homophily, and cross gender mentoring}
In addition, we used statistical tests to analyze the gender dimension for implicit mentoring from three aspects: comparison between proportions implicit mentoring given by men and women; comparison of homophily preferences of implicit mentoring between men and women; and comparison of cross-gender mentoring given by men with women. 




\subsection{Results}
Here we first discuss to what extent implicit mentoring occurs in our dataset and then characterize it through the type of mentoring interactions ($RQ \#2a$) and gender ($RQ \#2a$) lenses. 

\boldification{overall numbers show implicit mentoring is pervasive}
As a first step, we investigate how often implicit mentoring occurs via PR-comments. Our results show that a majority of PRs included implicit mentoring (67.53\% out of 974,44 PRs). A single PR can have multiple rounds of discussion between the PR-author and other developers, which is recorded via the PR-comments. In our dataset on an average a PR had 6.035 comments ($sd=8.054$). It is then possible that one or multiple of these comments could embed implicit mentoring. In our dataset a large portion of PR-comments embedded implicit mentoring (31.00 \%) and a majority of the developers provided such mentoring (70.73\% out of 11,634 developers). This shows that implicit mentoring is quite pervasive. Next, we characterize implicit mentoring further.





\subsubsection{Interaction Types in Implicit Mentoring (RQ \#2a)}
\label{flavors}

\begin{figure}[!tbp]
\centering
\includegraphics[width=3.5in]{pic/pr_mentoring.png}
\caption{PR-comments mentoring approaching}
\label{fig:PR}
\end{figure}







\boldification{Surprisingly...peer mentoring is the most common mentoring approach from our observations, within identified 67.583\% PRs contain implicit mentor, dyad (62.06\%): 40,837, triad (23.68\%): 15,585, >triad(14.26\%):9,383 }
%
Here we investigate to what extent implicit mentoring includes dyadic, top-down interactions ($RQ \#2a$).

We answer the first part of the question by considering the interactions for each PR. The PR-author is considered the mentee. Authors of PR-comments that included implicit mentoring are considered mentors. If the discussions occurred only between the mentee and one mentor, this mentoring is considered \textit{dyadic}. Similarly, if the discussions occur between an author and two mentors, its considered a triad. Finally, we group all mentee-mentor groups equal to or greater than four as $\ge$quadrad. Note, that for a PR, if there were other authors who commented, but were not mentors (comment was not considered mentoring), they are ignored in this analysis. 

Of the 65,805 PRs with implicit mentoring the majority was dyadic (62.06\%), lining up with the traditional view of mentor-mentee relationship. However, because of the open, voluntary-based  nature of OSS we found 23.68\% of mentoring occurring in triads and another 14.26\% in $\ge$quadrads. This is akin to ``it takes a village..." adage, where the community of developers work together to mentor developers and providing perhaps different perspectives and guidance.  

\begin{mdframed}[roundcorner=10pt]
  \textbf{Observation 1:} A majority of implicit mentoring is dyadic (62.6\%), but in a substantial number of cases (24,968 instances) multiple mentors provide support.
\end{mdframed}

Next, we investigate what role experience---within the project and overall---plays in implicit mentoring. There can be three types of mentoring directionality:
\begin{itemize}
    \item \textit{top-down}, the mentor is more experienced than the mentee,
    \item \textit{peer-to-peer}, the mentor and mentee have same level of experience,
    \item \textit{bottom-up}, mentee is more experienced than the mentor.
\end{itemize}

%
To obtain the direction of mentoring, we subtracted the first commit date of the mentee from that of the mentor. If the the difference is positive, then the PR-comment interaction is flagged as \textit{top-down} and if negative it is \textit{bottom-up}. If mentor and mentee had their first commits on the same day, then it is \textit{peer-to-peer}. 

Figure \ref{fig:PR} shows the distribution of these types of implicit mentoring when considering within the project (based on the first commit in the project, marked in blue) as well as overall experience, where we use the first commit by an author in GitHub as a proxy (yellow). 

About 31\% of implicit mentoring falls in the traditional top-down mentoring interaction style. The average difference between mentee and mentor experience was 608 days ($sd=567$). 10\% of implicit mentoring where in the bottom-up category with the mean difference between mentor-mentee being 361 days ($sd=444$).
The majority was in the peer-to-peer mentoring group---59\% accounting for 182,532 mentoring instances. 

One reason for this contradiction to the traditional view of top-down mentoring could be because in OSS, developers frequently contribute to multiple projects or migrate across projects~\cite{onion paper}. In such cases, they may accrue skills and experiences relevant to the project elsewhere. Therefore, we look at the mentoring directionality when considering the overall experience in GitHub. The results of this analysis was very similar to the within-project experience analysis, with the majority of implicit mentoring instances being peer-to-peer (59\%).
This was followed by \textit{top-down} mentoring (25\% of cases with mean difference in experience being 988 days ($sd=740$)) and \textit{bottom up} mentoring (16\%, mean difference being 842 days ($sd=676$)). 

When looking from the perspective of the developers who do mentoring, the story remains the same, with about 90\% of developers in our dataset having done peer-to-peer mentoring. 
This shows that “\textit{seniority is not necessary for implicit mentoring}” [P3]. 


\begin{mdframed}[roundcorner=10pt]
  \textbf{Observation 2:} Peer-to-peer mentoring is the most common form of implicit mentoring accounting for 59\% of cases, followed by top-down and bottom-up flavors of mentoring.
\end{mdframed}

\boldification{We identify gender through Namesor and tabel shows the distribution.}

\subsubsection{Gender Analysis of Implicit Mentoring}
To analyze implicit mentoring through the gender lens, recall, we used Namesor to identify the gender of contributors and only include those individuals for whom the API is able to predict gender with high confidence ($>90\%$).  In our data, we could identify the gender of 6,342 contributors. 


\input{Table/sec4_gender_overall}
Table \ref{tab:genderoverall} shows the distribution of developers in this dataset with respect to their gender and mentoring activity. 71.49\% of these developers acted as implicit mentors. That is, 4,534 developers were authors of least one PR-comment that was identified as implicit mentoring. Among these mentors, 5.30\% (240) were women and the 94.70\% (4,293) were men. 


\boldification{men doing more mentoring than women for overall mentoring approaches, but the effect size and estimated ratio are quite small, when we unpack, we noticed that women are doing more mentoring for bottom-up and top to down...}
\hl{Past research has shown that the conventional view of mentoring is women is doing more effective mentoring than men} \cite{sosik2000role}. 
To analyze whether there is any distinction between men and women with respect to the amount of mentoring they provide, we perform a proportion test (refer to ~\ref{sec:method}) between the proportions of men and women mentors. 
The results show that there is a significant difference ($estimate =.022, p<0.001$); men were 2.2\% times more likely to mentor than women.
The results indicate that men perform more mentoring than women, \hl{which is contrary to current perspective that women take up the primary burden of mentoring~}\cite{???}. 
%Yellow highlight means, AS needs to check if Lit supports this

\input{Table/sec4_gender_overall_Z}
One reason for this difference might be arising because our sample sizes are unequal. Therefore, we used estimated ratio and effect size to further investigate the differences between the groups. The estimated ratio of differences was small --- 0.022 (cf. Table \ref{tab:gender_overall_Z}). Next, we calculate effect size using Cohen's d \cite{cohen2013statistical}. The effect size of $d=0.048$ indicates that the differences between the proportion of mentoring by men and women are negligible. (Effect size thresholds of $d=0.2$ is considered small; $d=0.5$ medium, and $d=0.8$  large \cite{cohen2013statistical}).

\begin{mdframed}[roundcorner=10pt]
  \textbf{Observation 3:} More men than women provide implicit mentoring ($Estimate =.022, p<0.001$), but the effect size is negligible (Cohen $d=0.047$).
\end{mdframed}




Next, we investigate the different implicit mentoring approaches, such as peer-to-peer, bottom-up, top-to-down mentoring. Table XX presents the results of proportionality tests and the effect size.


When considering peer mentoring, more men than women were found to be implicit mentors ($estimate =.052, p<0.001$). However, the effect size is small (Cohen $d=0.112$). 
For top-down and bottom-up approaches too, we find significant difference between the proportion of mentoring given by women and men (Top$\rightarrow$Down: $estimate =-.098, p<0.001$, Bottom$\rightarrow$Up: $estimate =.022=-.032, p<0.001$). But, in both cases, the proportion of women was greater than that of men (and hence the negative value of the $estimate$-score). 
%For bottom-up, the proportion of mentoring for women was 0.028 more than men, and for top-to-down, it was 0.098 more than men. 
The effect sizes for bottom-up and top-to-down are 0.066 and 0.201, respectively. This implies that the effect sizes is negligible for bottom-up, and small for top-down mentoring. 

\begin{mdframed}[roundcorner=10pt]
  \textbf{Observation 4:} There are significant differences between men and women performing mentoring at the different levels, with men doing more peer-to-peer mentoring and women doing more top-down and bottom-up mentoring. In all cases, however, the differences is not large.
\end{mdframed}

%In summary, while there are significant differences between men and women performing implicit mentoring, the differences range from negligible to small.

%A possible reason may be because the sample size of peer mentoring is larger than other mentoring approaches, and it may have also affected the overall mentoring proportion test results.  

%\input{Table/sec4_chi2square}

\boldification{Our test indicates that for all identified implicit mentoring approaches, there are gender preferences when people give mentoring}

\input{Table/sec4_homophily_gender_dist}
Looking deeper into mentor-mentee relationships, our results indicate that gender preferences exist in implicit mentoring.
Table \ref{tab:gender_homophily_dist} presents the number of implicit mentoring comments for each pair of mentors and mentees, classified into the mentoring approach they took (bottom-up, top-to-down, peer mentoring). We used the $\tilde{\chi}^2$ test to understand the differences between the four pairs of mentor-mentee with respect to their gender (woman-woman, woman-man, man-woman, man-man). Our null hypothesis was all gender pairs of mentor and mentee are equally exists in implicit mentoring. %Our test results in Table \ref{tab:chi2} indicate that there is strong evidence indicating that at least one gender pair is different from the other for all mentoring approaches ($p<0.001$). Therefore, we can conclude that gender preferences exist for implicit mentoring in OSS. 


\input{Table/sec4_homophily_Z}
The other domain of research indicates that homophily preferences happen in mentoring \cite{kao2014should}.
Table \ref{tab:sec4_homophily_Z} indicates that there is strong evidence of the proportion of mentoring that happens between same-gender mentoring and cross-gender, and the estimated proportion ratio for all mentoring approaches are over 0.9, and effect size shows that the differences are remarkable for all mentoring approaches. 
Therefore, OSS developers are doing more homophily mentoring than non-homophily mentoring regardless of mentoring approaches.

%\input{Table/sec4_homophily_gender_diff-OLD}
\input{Table/sec4_homophily_gender_diff}
%\input{Table/sec4_homophil_cross_gender}

\boldification{women give more non-homophily than men for all mentoring approaches}
By studying the mentoring relationship regarding gender preferences, we continue study investigate proportion of each gender involve in homophily mentoring. Table 
%\ref{tab:pro_gender_samegender_OLD}
%\ref{tab:pro_gender_samegender} 
\ref{tab:pro_gender_samegender}


%shows the proportion test results of homophily preferences of each gender for implicit mentoring.
%There is strong evidence indicating that men are involving more homophily implicit mentoring than women for overall mentoring ($p<0.001$). When we unpack the mentoring approach, for top-to-down and bottom-up, we observe the proportion of homophily implicit mentoring happens in men is greater than in women, the estimated ratio for both cases are over 0.8, and effect size indicate the difference are remarkable. As for peer-peer mentoring, even we observe the estimated ratio is only 0.086, and the effect size indicates that the differences are still noticeable between men and women.  
  
Women are minority in OSS community \cite{canedo2020work}, which in line with our women mentors, we continue investigate which gender do more cross-gender mentoring. Table \ref{tab:pro_gender_samegender} presents the comparison results of non-homophily mentoring between men and women mentors. 
When we look at the overall mentoring approach, there is significant evidence indicating that men mentors give more implicit mentoring comments to women, the estimated ratio is 0.161, and the effect size is 0.624.
In addition, as for mentoring approach of bottom-up and top to down, the proportion of men homophily mentoring is greater than women, the estimated ratio and effect size are considerable as the effect size are over 1 for both mentoring approaches.
For peer mentoring, the results indicate a significant evidence men mentors doing more homophily mentoring than women, and the effect size is greater than 0.213. 
Therefore, men mentors give more homophily implicit mentoring across all mentoring approaches. 







==> OLD_IEEE/intro.tex <==
%!TEX root = main.tex

\section{Introduction}
\label{sec:intro}

\as{**Possible storyline [AS]***\\
**Mentoring is important for onboarding and future career growth, both in regular as well as OSS domains, and involves these things...

**But, mentoring has its own set of challenges, one of which is lack of visibility/ack. This lack of visibility can amount to mentors lose their engineering voice. Some research has shown that this is particularly true for women.

**When we unpack mentoring it can be explicit, but also implicit in the very activities that OSS devs do. for example....

**While explicit mentoring has been researched and roles are ack'ed, we dont know anything about implicit mentoring.

** Our goal is to understand how and to what extent (implicit) mentoring happens in day-to-day OSS dev tasks.

** To get to our goal we had to first understand what constitutes mentoring and the different flavors of mentoring. Leading to our first RQ: XXX. 

** To answer RQ1...we did Lit survey about different types of mentoring this way. We then did interviews this way. These gave us the def. of implicit mentoring:....

**The next question then is whether we can identify implicit mentoring, to understand to what extent this happens and who does it, bringing to our RQ2: XXX

**To answer RQ2, We did Data mining this way and identified 3 types of implicit mentoring

** we then did a distribution of the implicit mentoring by contributor demographics this way....

** Our contributions are:
1. a first investigation of implicit mentoring in OSS 
2. a mechanism to automatically identify implicit mentoring, that can help give visibility to contributors doing this
3. A characterization of the types and extent of implicit mentoring in a set of Apache projects}


\boldification{*** OSS projects are highly collaborative. To ensure successful project completion, mentoring is used widely in OSS for purposes like developing strategies, recommending tasks, etc.}
%
OSS (open-source software) projects are self-organized/organized and dynamic volunteers from all over the world contributing and collaborating \cite{de2019recommending, ducheneaut2005socialization, courant2006software, zhao2004user}. 
%
To ensure successful project completion, mentoring has been used widely in OSS for purposes including developing strategies, recommending tasks, helping new employees socialization, developing guidelines, applying strategies, and addressing issues \cite{balali2018newcomers, berlin1993beyond, sim1998ramp,steinmacher2012recommending, fagerholm2014role}.  
%
OSS organizations are providing systemic offline mentoring initiatives such as Google Summer of code \cite{lependu2020summer}. 



\boldification{**But, mentoring has its own set of challenges such as lacking of visibility/ack which can amount to mentors lose their engineering voice. Some research has shown that this is particularly true for women.}



\boldification{***When we unpack mentoring it can be explicit, but also implicit in the very activities that OSS developers do. For example, giving instructions, suggestions, comments, which are daily activities for developers in OSS. }

However, mentoring is not a one way in OSS,  which could have different forms based on different channels other than explicit/systemic mentoring \cite{fagerholm2014role}. 
%
Works of literature defined that mentoring is when a more experienced member from the organization providing guidance and suggestions for less experienced colleague to aid in organization socialization \cite{wilson1990organizational, awaya2003mentoring}. 
%
OSS developers are getting and giving comments frequently such as error-addressing, instructions and suggestions during developments regardless developers' background \cite{guzman2014sentiment, cseker2020new, datta2021understanding, steinmacher2014hard, steinmacher2012recommending, pehkonen2010mentoring}.
%
Thus, other than explicit/formal mentoring, OSS developers are getting mentored and mentoring others implicitly frequently. 



\boldification{***However, no research has investigated implicit mentoring in OSS.}

Past research shows that explicit mentoring is effective in offline and online OSS communities. There is no research on implicit mentoring in OSS.





\boldification{*** Therefore, to fill this gap, we investigate how and what extent (implicit) mentoring happens in daily OSS developers tasks. To guide our research, our goal is to understand what constitutes mentoring and the different flavors of mentoring.}
%
Therefore, our goal is to understand what constitutes mentoring and the different flavors of mentoring. 
%
To guide our research, this paper is focusing on the investigation of the following research questions:

RQ1. How do mentoring activities happen in OSS outside of formal mentoring?


RQ2. How to identify and characterize implicit mentoring?
%How much participants and who (gender dimension, experience dimension) are doing the implicit mentoring (peer to peer, top to down, down to top)? 


%RQ3. What are the benefits that implicit mentoring could bring to the OSS developers? 


\boldification{*** We first conduct a literature review and qualitative analysis on obtained responses from interviews. We find a gap that implicit mentoring have not been addressed from prior works. ***}
%
To investigate our research questions, we conduct literature review and qualitative analysis on obtained interview responses from professional OSS developers.
%
We find a significant gap that implicit mentoring and its benefits have not been addressed.


\boldification{*** To further identify implicit mentoring, we apply data mining on PR from GitHub projects since defined mentoring activities (instructions, suggestions) are giving while reviewing PR. And we apply machine learning methods to identify the implicit from mined data. ***}
%
To further identify implicit mentoring in OSS, we perform data mining on PR (Pull-request) from 37 Apache organizations on GitHub.
%
PR (Pull-Request) is an effective method on GitHub for review and management development contribution.
%
Comments, suggestions, and instructions are frequently giving while reviewing the PR \cite{zampetti2017developers,dey2020pull,yu2014reviewer}. 
%
We apply machine learning methods automatically identify the implicit mentoring from data we mined (107992 PR has been mined including 836,629 comments)


\boldification{*** In addition, we analyze our machine learning results to present the roles of characteristics for OSS implicit mentoring including experiences and gender.}
%
In addition, we analyzed the different roles of characteristics for OSS implicit mentoring such as experiences and gender.
%


\boldification{*** Our contributions are: 1. We first investigation of implicit mentoring in OSS, 2. We applied mechanism we learned to automatically identify implicit mentoring, that can help give visibility to contributors doing this. 3. A characterization of the types and extent of implicit mentoring in a set of Apache projects.}



This research contributes to the literature by (i) adding to the existing literature on the different mentoring forms during OSS development outside of formal mentoring; (ii) We applied mechanism we learned to automatically identify implicit mentoring, that can help give visibility to contributors doing this; (iii) presenting characterization of the types and extent of implicit mentoring in a set of OSS projects we collected.


 



==> OLD_IEEE/method.tex <==
\section{Methodology}
\label{sec:method}

\as{How about we refactor the section this way:}
\subsection{Defining Implicit Mentoring}
\textbf{Exploratory Interviews}

\textbf{Definition Validation}
- Member Checking
- Literature Survey

\subsection{Identifying Implicit Mentoring}
\textbf{Creating Training dataset}
- collecting Apache projects
- Manual labeling

\textbf{Building the classifier}
- details about the classifier
- details about gender classification

\as{the types of mentoring can be part of results...following the just in time principle}






\textbf{***Figure \ref{fig:rm} presents the overview of our research methodology in .}
%
The objective of this study is to investigate implicit mentoring in OSS, which involved 2 steps. First, we identified what implicit mentoring means for OSS and next we used data mining to identify implicit mentoring in OSS projects. 
%
First, we did an exploratory interview to.... invited 5 participants who are professional OSS developers and have more than 5 years of experience in the OSS community to participate in our interviews. 
%
We conducted interviews qualitative studies on obtained interview's responses.
%
We validated the findings from the interview through 2 steps. First, we did a literature survey of mentoring works. Second, we did a member checking with the interview participants.
%
\as{this next para is not connected to the prev one....need a transition}

In addition, to identify the implicit mentoring in OSS, our validation results indicated that PR comments from GitHub might be a place that implicit mentoring happens frequently. 
%
Therefore, we mined data for over 37 Apache projects on GitHub, comprising over 107,992 pull requests (PRs) and 836,629 PR comments.
%
Figure \ref{fig:rm} presents the overview of our research methodology. 
%
\begin{figure}[!tbp]
\centering
\includegraphics[width=3.4in]{pic/rm.png}
\caption{Research method overview}
\label{fig:rm}
\end{figure}




\subsection{Exploratory Interviews}
%
\as{most of this section is talking about explicit/implicit mentoring, have these terms been introduced already?...also need to mention if formal/informal mentoring are part of explicit?}
\textbf{***To investigate the implicit mentoring in OSS, we first interviewed 5 OSS experts this way. Table \ref{tab:demog} presents the demographic information of our participants}
%
To investigate the different flavors of mentoring we first interviewed 5 OSS experts.
%
We conduct structured interviews with OSS developers to investigate their understandings and experiences regarding the different types of mentoring they have experienced. We recruited OSS developers who has at least 5 years experiences working in OSS, and accepted referred participants by other interviewers, and ??not asked for further participants from referred participants???. 
%
The interviews were conducted remotely, lasting around 60 minutes each. Each interview was recorded with participants' consent (following university approved IRB protocol) and transcribed when the interview was over. Table \ref{tab:demog} presents the demographic information of our participants. Participants were offered \$50 gift card.
%
\begin{table}[!tbp]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|c|}{\textbf{Participant}}                               & \multicolumn{2}{c|}{\textbf{Years of experiences in}}                       & \multicolumn{4}{c|}{\textbf{Mentoring experiences}}                                                                                                                             \\ \hline
\multicolumn{1}{|c|}{\textbf{ID}} & \multicolumn{1}{c|}{\textbf{Gender}} & \multicolumn{1}{c|}{\textbf{OSS}} & \multicolumn{1}{c|}{\textbf{Mentoring}} & \multicolumn{1}{c|}{\textbf{Mentor}} & \multicolumn{1}{c|}{\textbf{Implicit/Explicit}} & \multicolumn{1}{c|}{\textbf{Mentee}} & \multicolumn{1}{c|}{\textbf{Implicit/Explicit}} \\ \hline
P1                                &                                      &                                   &                                         &                                      &                                                 &                                      &                                                 \\ \hline
P2                                &                                      &                                   &                                         &                                      &                                                 &                                      &                                                 \\ \hline
P3                                &                                      &                                   &                                         &                                      &                                                 &                                      &                                                 \\ \hline
P4                                &                                      &                                   &                                         &                                      &                                                 &                                      &                                                 \\ \hline
\end{tabular}}
\caption{Demographics}
\label{tab:demog}
\end{table}


At the beginning of the interview, we briefly explained to the participants the goals of the interviews and collect the demographic data. We asked participants about their roles and experiences in OSS, their mentoring experiences including both explicit and implicit, their understandings about implicit and explicit mentoring in OSS, benefits and impacts on their career.
%
To investigate definitions of implicit mentoring in OSS, our interview questions are formulated to investigate both implicit and explicit mentoring. We list the examples of some of the questions we asked during the interview, the full set of questions in the interview can be found on our site. 
\as{why only some of the questions? If these are the main mentoring related quesions then list all mentoring specific questions here...}
%
\as{these interview Q order seems odd...and it seems we are focusing on informal mentoring here...is that the same as implicit?}
- In your experience as a senior contributor how do you think formal and informal mentoring compare, where does one shine vs. other? 

- In this (OSS part of the) journey, where did you feel you got mentored?

- Did you get any informal mentoring in your journey?

- Did you informally mentor contributors in your journey?
%
\as{its odd to see this, usually there is a specific question...and not people just generally having a discussion...maybe, at the end we asked them for any other thoughts/feedback on mentoring and how to improve mentoring in OSS}
At the end of our interview, we allowed open-ended discussion about mentoring in OSS, participants shared their thinking from their mentoring experiences. 


\subsection{Literature survey}

\textbf{***To get an understanding of implicit mentoring, with the findings from the qualitative coding,  we conducted a literature survey.}
%
To get an understanding of implicit mentoring, with the findings from the qualitative coding, we conducted a literature survey. We found XX papers related to mentoring. Among the papers we found, x came from the field of OSS, xx came from the field of education, etc. (See Table XX)



\subsection{Expert validation}

\textbf{***Combing the findings from interviews and literature survey, we retrieved the definitions and typical activities to identify the implicit mentoring.}
%
Combing the findings from interviews and literature survey, we retrieved the definitions and typical activities to identify the implicit mentoring. To understand implicit mentoring in OSS from our interview raw data, we investigate our interview raw data from these aspects including: 1) activities of implicit mentoring; 2) benefits of implicit mentoring; 3) definition of implicit mentoring; 4) evaluations of implicit mentoring; 5) frequency of implicit mentoring; 6) channels of implicit mentoring; 7) reasons of implicit mentoring.  Section \ref{sec:result} presents our analysis results. 


\textbf{***To validate our findings, we complete a expert-validation survey. The survey consisted of 15 questions, including demographic questions and examples of PR comments from our dataset.}
%
To validate our findings, we complete a expert-validation survey. We sent the survey back to the people we have interviewed. The survey consisted of 15 questions, including demographic questions and examples of PR comments from GitHub. \cite{} and our interview analysis indicate that activities such as giving suggestions on code on PR channels are daily activities in OSS. Therefore, we chose PR-comments from GitHub to investigate the implicit mentoring.



Our survey was constructed with 15 questions, including yes/no, multiple-choice questions, and open-ended questions. Including demographic information, our survey is used to verify the definitions and activities of implicit mentoring we retrieved. In addition, to continue validating the understanding of implicit mentoring, we list 8 PR comments from GitHub and asked participants to identify whether it is implicit mentoring/not-mentoring. We have identified these PR comments based on retrieved definitions/activities before we deployed the survey. To the best of our understanding, there are 6 implicit mentoring, 2 non-mentoring comments. In the test run, the survey takes about five minutes to complete. The survey was conducted via Qualtrics. The full survey questions are found on our site. Figure \ref{fig:tv} presents the triangulation of our codeset with literature survey finding, interview transcripts, and expert validations.


\textbf{***Figure \ref{fig:tv} presents the triangulation of our codeset with literature survey finding, interview transcripts, and expert validations.}


\begin{figure}[!tbp]
\centering
\includegraphics[width=3.4in]{pic/tri_ver.png}
\caption{triangulation flow of our validation}
\label{fig:tv}
\end{figure}



\subsection{PR-comments data collection}
%
\textbf{We mined 37 Apache Projects on Github. Our dataset consisted of 107,992 Pull requests, and 836,729 comments.}
%
A random project selected from GitHub without a detailed record of the discussion program will be difficult to ensure that we have Identify all communication channels. Thus we chose the Apache project because they use Pull-requests as communication channel, and there are specific instructions for using PR-comments as communication channels. 

\zf{Apache is matured, structured.... in OSS community. }
%
In total, we have mined 836,729 comments of 107,992 Pull requests from 37 Apache projects. 



\subsection{Data analysis}
%
\textbf{***To find out who were participating in implicit mentoring and how, we had to identify mentoring comments within the PR. }
%
To find out who were participating in implicit mentoring and how, we had to identify mentoring comments within the PR. We applied the definitions and activities of implicit mentoring we retrieved to identify the implicit mentoring on PR-comments data we mined from GitHub. 
%
With large quantity of our datasets, it is impossible to identify the implicit mentoring manually, therefore, we decided to apply machine learning.



\textbf{***To train machine learning models, we first extract the samples to create the training dataset from 836,729 comments we mined with 95\% confidence intervals and a margin of error of 5\%.}
%
To train machine learning models, we first extract the samples to create the training dataset from 836,729 comments we mined with 95\% confidence intervals and a margin of error of 5\% \cite{kadam2010sample}. 
%

\textbf{***Two researchers separately coded on 20\% of samples and calculated IRR.}
Our sample has 384 PR-comments, to avoid personal subjective errors, two researchers separately coded on 20\% of samples and calculated Inter-Rater Reliability (IRR) \cite{hallgren2012computing}. 
%
94\% IRR had been obtained, the rest 80\% of the data samples were split and coded.



\textbf{***This coded data sample was our training dataset. Using this dataset, We applied 5 different machine learning methods with hyperparameter adjustments.}
%
Using samples we manually classified (implicit mentoring/not mentoring), We applied 5 different machine learning methods with hyperparameter adjustments.
%
Previous machine learning studies regarding text classification tasks have shown that classic supervised machine learning algorithms \cite{beyer2020kind, fu2017easy}. Thus, we have tested 5 different algorithms including Random Forest, Bernoulli, Support Vector, KNeighbors, and Decision trees. 
% 
After comparing the machine learning results, we chose the best performance model to help us identify the implicit mentoring for all the PR comments we mined. \ref{sec:result} presents the machine learning comparison results. 





\textbf{***To get a deeper  understanding of the mentor, we calculated the type of mentoring (peer-to-peer, top-to-down, bottom-up) based on their relative experience in the project. We have applied "Namsor" tool to identify the gender of mentor based on their geographic information}
% 
In addition, after categorizing classify the PR comments into implicit mentoring/not mentoring, we extract all of the implicit mentoring PR comments. 
%
To get a deeper  understanding of the mentor, we calculated the type of mentoring (peer-to-peer, top-to-down, bottom-up) based on their relative experience in the project and their GitHub experiences. 
%
In addition, We also identified their gender using the ``Namsor'' tool to identify the mentor's gender based on the geographic information they provided on GitHub. Previous research have proved the  `Namsor'' is a accurate tool to identify the gender based on their geographic  information\cite{jain2017location}.




==> OLD_IEEE/old.tex <==
\begin{comments}
Mentoring is important in open collaboration communities, particularly for onboarding and future career growth. 
Nevertheless, prior studies show that challenges exist in both formal and informal mentoring, which makes the mentoring system unstructured. 
Research so far has not looked at informal mentoring in OSS systemically, which has been proved more effective than formal mentoring in other domains.
Not recognizing informal mentoring may cause developers to lose their engineering voice.
While developers seek out informal mentors explicitly, there is another type of informal mentoring that happens in OSS during developers' day to day activities: implicit mentoring.


Since little is known about implicit mentoring in OSS, in our work, we interviewed OSS developers who have both formal/informal experiences and qualitatively analyzed their answers.
We retrieved the definitions of implicit mentoring in OSS by validated our findings with a literature survey and member check survey. 
Additionally, we mined Pull-request (PR) with comments from 37 Apache projects as PR is one of identified channels that implicit mentoring happens in OSS.
We are able to automatically identify implicit mentoring using a supervised machine learning classifier.
By quantitatively analyze identified implicit mentoring data, the majority of PRs include implicit mentoring (67.58\%).
Interestingly, over half of implicit mentoring happens in peer-to-peer mentoring approaches. 
Since gender-related challenges emerged in our analysis, our gender-related quantities analysis shows that homophily preferences are the majority mentoring relationships in OSS. Moreover, women mentors provide more cross-gender mentoring.

The contributions of this paper include:
defining the implicit mentoring in OSS; 
Automatically identifying implicit mentoring;
investigating seniority and gender characteristic of implicit mentoring. 
Online communities, organizations, can leverage this knowledge to foster more mentoring to OSS projects.
\end{comments}

==> OLD_IEEE/related.tex <==
%!TEX root = main.tex

\section{Related Work}
\label{sec:relatedwork}
 \as{new outline for RW}
 
 **mentoring has been investigated in Management lit as well as SE...examples
 
  **Mentoring in OSS has been talked about this way.
 
 **one form of mentoring is implicit mentoring, defined as this...by these people...and shown to be helpful....
 
 **Implicit mentoring in the SE domain as been talked this way...nothing about implicit mentoring in the OSS domain
 

\boldification{People have talked about mentoring in several domains.}
\hl{write 1 to 2 sentences about the key findings in these papers. Allen...relationship between mentoring and positive org. attitudes. They found mentoring to improve org commitments, etc etc. etc.}
Mentoring has been thoroughly researched in various domains. In management and organizational literature, works have investigated the extent that employees learn helping behaviours from mentors~\cite{eby2015cross}. They found that mentoring received was positively associated with employee inter-personally oriented organizational citizenship behavior (OCB). Payne et al. investigated the relationship between mentoring and positive organizational attitudes and their findings indicated that mentoring was positively related to affective commitment and continuance commitment but negatively related to turnover behaviour~\cite{payne2005longitudinal}. Similarly, in education literature, Mullen et al. conducted a literature review of empirical studies on mentoring to define comtemporary mentoring and explore relevant types and applications~\cite{mullen2021defining}.

\boldification{One form of mentoring is implicit mentoring.}
One form of mentoring is informal mentoring. According to Inzer et al.~\cite{inzer2005review}, informal mentoring occurs in a relationship between two people where one gains insight, knowledge, wisdom, friendship, and support from the other. Cotton and Ragins found that informal mentoring is more beneficial than formal mentoring as the former provided higher amounts of career development functions such as: coaching, providing challenging assignments, or increasing exposure and visibility of the mentee. Their findings showed that mentees who were informally mentored were much more satisfied with their mentors than mentees with formal mentors~\cite{ragins1999mentor, inzer2005review,bynum2015power}. Inzer et al. states that informal mentoring is a valuable tool for developing an employee as it occurs in a relationship that is voluntarily formed by both persons. It is friendship first, learning and career second and third. Similarly, in education literature, Seery et al. focused on the peer mentoring among students as partners and found that peer mentors not only developed new skills and relationships but also their friendships and networks significantly expanded~\cite{seery2021students}. 
\ac{addressed} \as{do they have a formal definition of this? Give some examples that were put in the paper}

\boldification{SE has defined mentoring in these ways.}
Software Engineering research has also investigated mentoring, specially in onboarding activities. For example, Google has tried to improve the onboarding process using mentorship programs~\cite{johnson2010learning}. In OSS, researchers looked at the role of mentoring for onboarding to OSS projects where they found that developers receiving onboarding support were
more efficient and effective than developers who entered the same
projects through the natural, non-deliberate process~\cite{fagerholm2014role}. Kumar et al. investigated communication strategies for mentoring in software development projects, such as interrogation, where the mentor asks a question typically followed by advice or sharing of strategies to overcome the identified problem. 
There are only two papers clearly addressed the implicit mentoring for software engineering and computing area, but limited with teen learners. Ko et.al \cite{ko2018informal} addressed that implicit mentoring relationship is significantly effective for teen learners in computing. Nandi and Mandernach \cite{nandi2016hackathons} concluded that students are heavily motivated by informal mentoring relationship. Analysis from surveys, student academic records and source-code commit log data shows that students grows significantly due to the implicit mentoring. However, none of the works have explored implicit mentoring among developers in OSS. Our paper fills this gap by investigating how implicit mentoring happens in OSS and who are these mentors in the OSS community.





% \as{not seeing how the following para is related work to mentoring}
% Tan et. al \cite{tan2021github} find that the GitHub, as one of the most popular OSS community, ensure the code quality by using mentors to review codes. And these activities are not limited to explicit mentoring.  
% Hayashi et.al \cite{hayashi2013collaboration} address that singly developer in OSS always only has narrow knowledge, collaborations is one of the methods to over difficulties. For example,  if one committer does not have sufficient knowledge of related parts, collaborations must be taken place to verify and commit the bug-fix. This process can be identified as implicit mentoring, since the collaboration can happens randomly, but the the process including addressing issues, giving instructions, etc. 




% OBSOLETE below: 
% In this section, we present existing works on OSS mentoring, implicit mentoring in OSS, and gender diversity of the mentoring. 



% \textbf{***To get to our goal we had to first understand what constitutes mentoring and the different flavors of mentoring, we first applied literature survey on mentoring in OSS.}
% %
% To get to our goal we had to first understand what constitutes mentoring and the different flavors of mentoring research in the field of OSS mentoring, we conduct a literature survey. 
% %
% We focus on the papers from 2012 to 2021 (inclusive) that related to mentorship in top conferences in Software Engineering: IEEE-ICSME, IEEE-RSSE, IEEE-ICGSEW, ACM-FSE, ACM-ESEM, ACM-ICSE, IEEE-ICSME, IEEE-MSR, ACM-SIGCSE, ACM-HCI, and ACM-ICPS.
% %
% While conducting the literature survey, we searched for a set of keywords including mentoring in OSS, mentorship in OSS, implicit mentoring in OSS, informal mentoring software engineer etc. We found 23 papers on mentoring in OSS. And Table \ref{tab:literaturesurvey} presents the summary of the literature survey for most recent 10 years. 


% \subsection{Implicit mentoring in OSS}
% \as{confused about this sub section, its already discussed no?}
% %
% Understanding implicit mentoring in the OSS community is particularly relevant for OSS developers, organizations, and researchers to have a broader view of mentoring.


% Tan et. al \cite{tan2021github} find that the GitHub, as one of the most popular OSS community, ensure the code quality by using mentors to review codes. And these activities are not limited to explicit mentoring.  
% Hayashi et.al \cite{hayashi2013collaboration} address that singly developer in OSS always only has narrow knowledge, collaborations is one of the methods to over difficulties. For example,  if one committer does not have sufficient knowledge of related parts, collaborations must be taken place to verify and commit the bug-fix. This process can be identified as implicit mentoring, since the collaboration can happens randomly, but the the process including addressing issues, giving instructions, etc. 


% There are only two papers clearly addressed the implicit mentoring for software engineering and computing area, but limited with teen learners. Ko et.al \cite{ko2018informal} addressed that implicit mentoring relationship is significantly effective for teen learners in computing area after analyzed from obtained interviews results. Nandi and Mandernach \cite{} conclude that students are heavily motivated by the informal mentoring relationship. Analysis from surveys, student academic records and source-code commit log data shows that students grows significantly due to the implicit mentoring. 



% \subsection{Gender diversity}
% \textbf{What is the role of diversity in mentoring?}

% Work of literature indicates that implicit mentoring relationship happens in peer to peer frequently. There is no research mentioned the gender diversity of mentoring in OSS community, especially implicit mentoring. 
% %
% Athey et al. stated that mentoring happens more when the mentors and protege are of same-gender \cite{athey2000mentoring}. 
% %
% In addition, Neill addressed that mentoring for the role of gender increased significantly \cite{o2012gender}.
% %
% Cross-gender mentorship becomes a challenge in their workplace that may limit individual growth, group productivity, etc \cite{mckeen2007gender}

% However, in the OSS community, Vasilescu et al. stated that gender diversity has a significant positive for productivity \cite{vasilescu2015gender}. 
% %
% In addition, female developers in the OSS community are facing more barriers but less ambitious and competitive than men \cite{balali2018newcomers}. 
% %
% Thus, understanding the gender diversity for mentoring in the OSS community, especially for implicit mentoring would inform decisions to lead better team organizations, recruiting, and productivity. 



% \subsection{Section remarks}
% Studies show that mentoring is an effective way to support OSS developers and improve productivity in OSS projects.
% %
% However, none of them identified the channels of mentoring in OSS communities. 
% %
% What is more, numerous studies presents the definition of mentoring in OSS, no literature investigates how does implicit mentoring contribute to the OSS community.
% %
% In addition, our contribution also presents evidence on the role of gender in implicit OSS mentoring. 



==> OLD_IEEE/results.tex <==
%!TEX root = main.tex

\section{Results}
\label{sec:result}

In this section, we present the results of our investigations structured by our research questions. 

\subsection{RQ1. How  do  mentoring  activities  happen  in  OSS  outside of the formal assigned mentoring?}



\textbf{***To validate our findings from our qualitative analysis on obtained interviews, we conducted literature survey. After qualitative analysis on obtained interview transcripts and quantitative analysis on expert validation survey, we find: 1. implicit mentoring happens frequently in OSS developer's daily activities; 2. Code reviewing is one such that typical activities which involves, error addressing, instruction/suggestions providing, etc.; 3.Figure \ref{} presents the definition of implicit mentoring in OSS we retrieved.}


\as{this is all about method...what needs here is a table of definition of implicit mentoring}
To answer our first research question, we did a qualitative analysis on obtained interviews and literature survey to identify papers on mentoring. We found the definitions that they used and retrieved the actions that qualify as mentoring in OSS, such as "Addressing errors", "giving suggestions" and "providing instructions". Based on this, we made a codeset which defined mentoring as either of these three activities. To understand more about implicit mentoring, we conducted interviews with industry experts and validated our findings from the literature survey with a expert validation survey, in which we asked them if they agreed with our definitions and their opinions on PR comments on whether they were considered to be mentoring or not and the reasoning behind it.

\as{this part needs more meat....some quotes...where informal mentoring shines...etc.}

\as{then present the results of triangulation (table) with the def. triangulation; we may talk about how we did triangulation here instead of method...not sure yet}

\as{this present results on the classification of implicit mentoring...the binary one}

\as{based on survey results, we can also put some data if the PR comments we picked were verified...a union of all answers is ok}






\subsection{RQ2. what are the characteristics of implicit mentoring: a) who does it, b) how often it happens, c) what level?}
%How many participants and who (gender dimension, experience dimension) are doing the implicit mentoring (peer to peer, top to down, down to top)?}

\textbf{***To answer this research question, we first mined Pull-request data from 37 Apache repos from GitHub} \as{already in method}

In total, we have mined 107,992 Pull Requests (PR), note that insides these PRs, there are a total of 836,729 comments.

\textbf{***To identify the implicit mentoring from the PR-comments, we used the codesets we investigated from RQ1.  }

\textbf{***However, it is impossible to identify the implicit mentoring from 107,992 pull requests. Therefore we applied machine learning to help us identify the implicit mentoring automatically.}

\textbf{***To train our machine learning models, we first randomly extract 338 PR-comments samples. Two researchers have identified implicit mentoring separately after cross validation.} \as{the classification building should be in method}

\textbf{***To obtain the best machine learning models, we have applied 5 different machine learning models, table presents the machine learning comparison results.}

\textbf{***After applying the Random forest classifier, we have identified *** number of implicit mentoring PR-comments. }

\textbf{***By applying ''Namsor" gender identification API, we identified that \% of implicit mentoring are giving by the female, and the plot below shows the distribution of the gender.}

\textbf{***What is more, to understand the role of characteristics of implicit mentoring other than gender, we conduct quantitative analysis on level dimensions from identified mentoring}

\textbf{***There two types of experiences of each PR-comments author, within the project they have been working on and overall GitHub experiences. }

\textbf{***We grouped identified each implicit mentoring PR comments into three categories i.e peer to peer, top to down, and down to top.}

\textbf{***Figure \ref{} and \ref{} presents the our experience results. } 







==> OLD_IEEE/sec3_challenge_table.tex <==
\begin{table}[tbp]
\caption{Challenge table}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|llll}
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{000000} \textbf{}}                                                                                                                               & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{Challenge name}}}                       & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{Sample quote}}}                                                                                                                         & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Mentioned \\ by\end{tabular}}}} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{Literature}}}                                                                                                                        \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }}                                                                                           & {\color[HTML]{000000} Hard to find a mentor}                                                                     & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P1:"I always have trouble \\ getting mentors "\end{tabular}}                                                                                                    & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P1,P2,\\P3, P5\end{tabular}}                                                     & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}\cite{steinmacher2014hard, steinmacher2015systematic}\\ \cite{trinkenreich2021women, balali2020recommending}\end{tabular}} \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Mentoring \\ in general\end{tabular}}}}} & {\color[HTML]{000000} Return on investment}                                                                      & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P2:"It's hard to assess \\ during the mentorship\\ whether the return on \\ investment is going to\\ be effective.\end{tabular}}                                & {\color[HTML]{000000} P2,P5}                                                                                                       & {\color[HTML]{000000} \cite{silva2017long}}                                                                                                                                                  \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                                                                                                & {\color[HTML]{000000} Diverging interests}                                                                       & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P5:"Your interests tend \\ to diverge, you tend to \\ look for new mentors, \\ new areas, and new\\ people to serve."\end{tabular}}                             & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P3,P4,\\P5\end{tabular}}                                                        & {\color[HTML]{000000} \cite{balali2018newcomers, balali2020recommending}}                                                                                                                    \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                                                                                                & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Too overwhelming to \\ navigate being \\ a mentee\end{tabular}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P4:"I really got \\ overwhelmed with \\ all the information. \\ And I didn't have \\ many ideas what to\\ ask for my mentor \\ to guide me with."\end{tabular}} & {\color[HTML]{000000} P2,P4}                                                                                                       & {\color[HTML]{000000} \cite{balali2020recommending,  steinmacher2014hard}}                                                                                                                   \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                                                                                                & {\color[HTML]{000000} Limited resources}                                                                         & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P5:"We basically \\ had raised enough \\ funding for having \\ a full-time position."\end{tabular}}                                                             & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P1,P2,\\P5\end{tabular}}                                                        & {\color[HTML]{000000} \cite{silva2020google}}                                                                                                                                                \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}l@{}}Formal \\ mentoring\end{tabular}}}}                          & {\color[HTML]{000000} Following through}                                                                         & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P4:"There was no \\ continuous progress of\\ mentoring, we didn't \\ know how to follow\\ up on things."\end{tabular}}                                          & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P1,P3,\\P4\end{tabular}}                                                        & {\color[HTML]{000000} \cite{balali2020recommending, steinmacher2015social}}                                                                                                                  \\ \hline

\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}l@{}}Informal \\ mentoring\end{tabular}}}                                          & {\color[HTML]{000000} unrecognized}                                                                              & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P2:" I leave the employee\\ doesn't have any recognition \\ for this mentorship."\end{tabular}}                                                                 & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P2,P3,\\P4, P5\end{tabular}}                                                    & {\color[HTML]{000000} \cite{steinmacher2021being}}                                                                                                                                          
\end{tabular}}                                                         
\label{tab:challenge}
\end{table}


==> OLD_IEEE/sec3_mentoring_type.tex <==
\begin{table}[!tbp]
\caption{Different flavor of mentoring}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll}
\rowcolor[HTML]{EFEFEF} 
\textbf{Mentoring} & \begin{tabular}[c]{@{}l@{}} ``A relationship between a less experienced individual,\\
called a mentee or protégé, and a more experienced\\ individual known as a mentor.  \cite{wai2009definition}\end{tabular}                                                                                                      \\
\textbf{Informal}  & \begin{tabular}[c]{@{}l@{}} ``Informal mentoring is the natural coming together of a \\mentor and protégé." \cite{inzer2005review}\end{tabular}                                                                                            \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Formal}    & \begin{tabular}[c]{@{}l@{}} ``Formal mentoring relationship are those that are initiated \\ through some organizational program that assigns mentors\\ and protégé" \cite{baugh2007formal}\end{tabular} \\
\textbf{Explicit}  & \begin{tabular}[c]{@{}l@{}} ``protégés expect and desire a relationship with a mentor who \\provides explicit direction and guidance," \cite{noonan2007peer}\end{tabular}                                        \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Implicit}  & \begin{tabular}[c]{@{}l@{}}Informal based relationship  between \\companies implicitly support others among daily activities.\end{tabular}                                                                                         
\end{tabular}}
\label{tab:mentoring_type}
\end{table}



==> OLD_IEEE/sec3_participant_demo.tex <==
\begin{table}[!tbp]
\caption{Demographic information our interview participants}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lll|llll|}
                                                 &                                                    &                          & \multicolumn{4}{c|}{\textbf{Mentoring experiences}}                                                                                                                           \\ \hline
\multicolumn{1}{|l|}{\textbf{ID}}                & \multicolumn{1}{l|}{\textbf{Gender}}               & \textbf{OSS experiences} & \textbf{Mentor} & \textbf{\begin{tabular}[c]{@{}l@{}}Informal\\ /Formal\end{tabular}} & \textbf{Mentee} & \textbf{\begin{tabular}[c]{@{}l@{}}Informal\\ /Formal\end{tabular}} \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}P1} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}Woman} & Over 10 years            & Y               & Both                                                                & Y               & Both                                                                \\
\multicolumn{1}{|l|}{P2}                         & \multicolumn{1}{l|}{Man}                           & Over 10 years            & Y               & Both                                                                & Y               & Both                                                                \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}P3} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}Woman} & 6-10 years               & Y               & Both                                                                & Y               & Both                                                                \\
\multicolumn{1}{|l|}{P4}                         & \multicolumn{1}{l|}{Woman}                         & 6-10 years               & Y               & Both                                                                & Y               & Both                                                                \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}P5} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}Woman} & 6-10 years               & Y               & Both                                                                & Y               & Both                                                               
\end{tabular}}
\label{tab:participant_demo}
\end{table}


==> OLD_IEEE/sec3_valid_table.tex <==
\begin{table}[!tbp]
\caption{Validation Table of Implicit mentoring}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllll}
\multicolumn{1}{c}{}                                                                                         & \multicolumn{1}{c}{}                                                       & \multicolumn{3}{c}{\textbf{Provenance}}                                                                                                                                                                 \\ \cline{3-5} 
\multicolumn{1}{c}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Implicit \\ mentoring\end{tabular}}}} & \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Items}}}                       & \textbf{Interview} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Literature \\ survey\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Member \\ checked\end{tabular}}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                     & Suggestions                                                                & P1, P3, P5         &\cite{ko2018informal, balali2018newcomers, trinkenreich2020hidden,fagerholm2014onboarding, zhou2012make}                                                                                           &\checkmark                                                                                        \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                     & Instructions                                                               & P2, P3, P4, P5     &\cite{ko2018informal, balali2018newcomers, trinkenreich2020hidden,fagerholm2014onboarding, zhou2012make}                                                                                          &\checkmark                                                                                         \\
\rowcolor[HTML]{EFEFEF} 
\multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Activities}}                                                & Addressing errors                                                          & P1,P3, P5          &\cite{ko2018informal, balali2018newcomers, bosu2019diversity, fagerholm2014onboarding, zhou2012make}                                                                                           &\checkmark                                                                                         \\ \hline
                                                                                                             & Email                                                                      & P1, P3, P4, P5     &\cite{balali2018newcomers, zhou2012make}                                                                                           &\checkmark                                                                                         \\
                                                                                                             & \begin{tabular}[c]{@{}l@{}}Code review tool \\ (e.g PR-comments)\end{tabular} & P1, P3, P4         &\cite{balali2018newcomers, trinkenreich2020hidden, bosu2019diversity, fagerholm2014onboarding, zhou2012make}                                                                                           &\checkmark                                                                                         \\
\multirow{-3}{*}{\textbf{Channels}}                                                                          & In person/Remote                                                           & P1, P4, P5             &\cite{ko2018informal}                                                                                           &\checkmark                                                                                        \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Frequency}                                                                                           & Everyday activities                                                        & P1, P2, P3, P4, P5 & \cite{ko2018informal, balali2018newcomers}                                                                                            &\checkmark &                                                                          
\end{tabular}}
\label{tab:val_tab}
\end{table}

==> OLD_IEEE/sec4_chi2square.tex <==
\begin{table}[!tbp]
\caption{$\tilde{\chi}^2$ test results of homophily preferences}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lll}
                                                                                                                & \textbf{Results}                                                                                                                                                              & \textbf{P-value (chi square )}                                     \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                        & \cellcolor[HTML]{EFEFEF}                                                                                                                                             & \cellcolor[HTML]{EFEFEF}                                   \\
\cellcolor[HTML]{EFEFEF}                                                                                        & \cellcolor[HTML]{EFEFEF}                                                                                                                                             & \cellcolor[HTML]{EFEFEF}                                   \\
\multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}l@{}}Overall\end{tabular}}} & \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}At lesat one of the group is \\ different than others in Table \ref{tab:gender_implicit}\end{tabular}} & \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\textless{}0.001} \\
                                                                                                                &                                                                                                                                                                      &                                                            \\
\multirow{-2}{*}{\textbf{Top$\rightarrow$Down}}                                                                            & \multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}At lesat one of the group is \\ different than others in Table \ref{tab:gender_implicit}\end{tabular}}                         & \multirow{-2}{*}{\textless{}0.001}                         \\
\cellcolor[HTML]{EFEFEF}                                                                                        & \cellcolor[HTML]{EFEFEF}                                                                                                                                             & \cellcolor[HTML]{EFEFEF}                                   \\
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Peer$\rightarrow$Peer}}                                                  & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}At lesat one of the group is \\ different than others in Table \ref{tab:gender_implicit}\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textless{}0.001} \\
\textbf{Bottom$\rightarrow$Up}                                                                                         & \begin{tabular}[c]{@{}l@{}}At lesat one of the group is \\ different than others in Table \ref{tab:gender_implicit}\end{tabular}                                           & $<0.001$                                          
\end{tabular}}
\label{tab:chi2}
\end{table}

==> OLD_IEEE/sec4_gender_overall.tex <==

\begin{table}[!tbp]
\caption{Summary of implicit mentoring gender}
\resizebox{\columnwidth}{!}{
\begin{tabular}{llll}
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{000000} \textbf{}}        & {\color[HTML]{000000} \textbf{women}} & {\color[HTML]{000000} \textbf{men}} & {\color[HTML]{000000} \textbf{Total}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Total developers}               & 353 (5.57\%)                                   & 5,989 (94.43\%)                              & 6,342                                 \\
\textbf{Implicit mentors}               & 240 (5.30\%)                                   & 4,293 (94.70\%)                               & 4,533                                 \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Total number of PR-comment}     & 8,581 (2.62\%)                                  & 318,546 (97.38\%)                             & 327,127                               \\
\textbf{Implicit mentoring PR-comments} & 2,745 (2.46\%)                                & 108,908 (97.54\%)                            & 111,653                              
\end{tabular}}
\label{tab:genderoverall}
\end{table}

==> OLD_IEEE/sec4_gender_overall_Z.tex <==

\begin{table}[!tbp]
\caption{Proportion test comparing implicit mentoring provided by men vs. women.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllll}
                                                                               & \textbf{Overall} & \textbf{Top$\rightarrow$Down} & \textbf{Peer$\rightarrow$Peer} & \textbf{Bottom$\rightarrow$Up} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Proportion Z-test}                                                 & P1 $\neq$ P2     & P1 $\neq$ P2         & P1 $\neq$ P2            & P1 $\neq$ P2       \\
\textbf{P-value}                                                               & \textless{}0.001 & \textless{}0.001     & \textless{}0.001        & \textless{}0.001   \\
\rowcolor[HTML]{EFEFEF} 
\textbf{\begin{tabular}[c]{@{}l@{}}Estimated ratio\\ differences\end{tabular}} & 0.022            & -0.098               & 0.052                   & -0.032             \\
\textbf{Effect size}                                                           & 0.047            & 0.202                & 0.112                   & 0.066              \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{l}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}P1: proportion of mentoring given by men\\ P2: proportion of mentoring given by women\end{tabular}}      
\end{tabular}}
\label{tab:gender_overall_Z}
\end{table}

==> OLD_IEEE/sec4_homophil_cross_gender.tex <==
\begin{table}[!t]
\caption{Proportion test results of cross-gender mentoring}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllll}
                                                                                 & \textbf{Overall}   & \textbf{Top$\rightarrow$Down}   & \textbf{Peer$\rightarrow$Peer}  & \textbf{Bottom$\rightarrow$Up}  \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Proportion Z-test}                                                       & P1 $\neq$ P2       & P1 $\neq$ P2           & P1 $\neq$ P2             & P1 $\neq$ P2        \\
\textbf{P-value}                                                                 & \textless{}0.001   & \textless{}0.001       & \textless{}0.001         & \textless{}0.001    \\
\rowcolor[HTML]{EFEFEF} 
\textbf{\begin{tabular}[c]{@{}l@{}}Estimated ratio\\ differences\end{tabular}}   & -0.161             & -0.440                 & -0.022                   & -0.750              \\
\textbf{Effect size}                                                             & 0.624              & 1.163                  & 0.213                    & 1.843               \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{l}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}P1:Proportion of non-homophily mentoring provided by men mentor (m$\rightarrow$w/(m$\rightarrow$m + m$\rightarrow$w))\\ P2:Proportion of non-homophily mentoring provided by women mentor (w$\rightarrow$m/(w$\rightarrow$w + w$\rightarrow$m)\end{tabular}}
\end{tabular}}
\label{tab:sec4_homophil_cross_gender}
\end{table}

==> OLD_IEEE/sec4_homophily_Z.tex <==
\begin{table}[tbp]
\caption{Proportion test results of homophily preferences }
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllll}
                                                                                    & \textbf{Overall}     & \textbf{Top$\rightarrow$Down}     & \textbf{Peer$\rightarrow$Peer}     & \textbf{Bottom$\rightarrow$Up}     \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Proportion Z-test}                                                          & P1 $\neq$ P2         & P1 $\neq$ P2             & P1 $\neq$ P2                & P1 $\neq$ P2           \\
\textbf{P-value}                                                                    & \textless{}0.001     & \textless{}0.001         & \textless{}0.001            & \textless{}0.001       \\
\rowcolor[HTML]{EFEFEF} 
\textbf{\begin{tabular}[c]{@{}l@{}}Estimated ratio\\ differences\end{tabular}}      & 0.964                & 0.930                    & 0.994                       & 0.920                  \\
\textbf{Effect size}                                                                & 2.600                & 2.390                    & 2.918                       & 2.331                  \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{l}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}P1:Proportion of mentoring given by same gender ((m$\rightarrow$m + w$\rightarrow$w) / All mentoring)
\\ P2:Proportion of mentoring given by different gender ((m$\rightarrow$w + w$\rightarrow$m) / All mentoring)\end{tabular}}
\end{tabular}}
\label{tab:sec4_homophily_Z}
\end{table}


==> OLD_IEEE/sec4_homophily_gender_diff-OLD.tex <==
\begin{table}[!t]
\caption{Proportion test results of homophily preferences for each gender}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllll}
                                                                                 & \textbf{Overall}   & \textbf{Top$\rightarrow$Down}   & \textbf{Peer$\rightarrow$Peer}  & \textbf{Bottom$\rightarrow$Up}  \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Proportion Z-test}                                                       & P1 $\neq$ P2       & P1 $\neq$ P2           & P1 $\neq$ P2             & P1 $\neq$ P2        \\
\textbf{P-value}                                                                 & \textless{}0.001   & \textless{}0.001       & \textless{}0.001         & \textless{}0.001    \\
\rowcolor[HTML]{EFEFEF} 
\textbf{\begin{tabular}[c]{@{}l@{}}Estimated ratio\\ differences\end{tabular}}   & 0.454              & 0.807                  & 0.086                    & 0.846               \\
\textbf{Effect size}                                                             & 1.243              & 1.946                  & 0.493                    & 2.048               \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{l}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}
%NEW: P1:Proportion of homophily mentoring of men (m$\rightarrow$m/ (m$\rightarrow$w + m$\rightarrow$m))\\ 
%NEW:P2:Proportion of homophily mentoring of women men (w$\rightarrow$w/ (w$\rightarrow$m + w$\rightarrow$w)\end{tabular}}

OLD: P1:Proportion of homophily mentoring of men (m$\rightarrow$m/ (m$\rightarrow$w + m$\rightarrow$m + w$\rightarrow$m))\\ 
OLD: P2:Proportion of homophily mentoring of women men (w$\rightarrow$w/ (w$\rightarrow$m + w$\rightarrow$w + m$\rightarrow$w)\end{tabular}}
\end{tabular}}
\label{tab:pro_gender_samegender_OLD}
\end{table}






==> OLD_IEEE/sec4_homophily_gender_diff.tex <==
\begin{table}[!t]
\caption{Proportion test results of homophily preferences for each gender}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllll}
                                                                                 & \textbf{Overall}   & \textbf{Top$\rightarrow$Down}   & \textbf{Peer$\rightarrow$Peer}  & \textbf{Bottom$\rightarrow$Up}  \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Proportion Z-test}                                                       & P1 $\neq$ P2       & P1 $\neq$ P2           & P1 $\neq$ P2             & P1 $\neq$ P2        \\
\textbf{P-value}                                                                 & \textless{}0.001   & \textless{}0.001       & \textless{}0.001         & \textless{}0.001    \\
\rowcolor[HTML]{EFEFEF} 
\textbf{\begin{tabular}[c]{@{}l@{}}Estimated ratio\\ differences\end{tabular}}   & 0.161              & 0.440                 & 0.022                    & 0.750               \\
\textbf{Effect size}                                                             & 0.624              & 1.171                  & 0.213                    & 1.841               \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{l}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}
NEW: P1:Proportion of homophily mentoring by men (m$\rightarrow$m/ (m$\rightarrow$w + m$\rightarrow$m))\\ 
NEW:P2:Proportion of homophily mentoring by women (w$\rightarrow$w/ (w$\rightarrow$m + w$\rightarrow$w)\end{tabular}}

%P1:Proportion of homophily mentoring of men (m-m/ (m-w + m-m + w-m))\\ 
%P2:Proportion of homophily mentoring of women men (w-w/ (w-m + w-w + m-w)\end{tabular}}
\end{tabular}}
\label{tab:pro_gender_samegender}
\end{table}





==> OLD_IEEE/sec4_homophily_gender_dist.tex <==
\begin{table}[tbp]
\caption{Implicit mentoring gender information ADD \% for each cell}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllll}
                         & \textbf{Overall} & \textbf{Top$\rightarrow$Down} & \textbf{Peer$\rightarrow$Peer} & \textbf{Bottom$\rightarrow$Up} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{W$\rightarrow$W} & 2,265                      & 258                  & 1,947                   & 60                 \\
\textbf{W$\rightarrow$M} & 480                        & 228                  & 48                      & 204                \\
\rowcolor[HTML]{EFEFEF} 
\textbf{M$\rightarrow$W} & 1,551                      & 1146                 & 143                     & 262                \\
\textbf{M$\rightarrow$M} & 107,794                    & 37,676              & 59,029                  & 11,089              \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Total}           & 112,090                    & 39,308              & 61,167                  & 11,615             
\end{tabular}}
\label{tab:gender_homophily_dist}
\end{table}

==> OLD_IEEE/sec4_ml_results.tex <==
\begin{table}[tbp]
\caption{precision, recall, F1, and AUC for classifiers}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllll}
\textbf{}             & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{AUC} \\ \hline
\rowcolor[HTML]{B4DAB4} 
\textbf{RandomForest} & 0.844              & 0.905           & 0.874       & 0.905        \\ \hline
\textbf{NaiveBayes}   & 0.837              & 0.857           & 0.847       & 0.897        \\ \hline
\textbf{SVM}          & 0.841              & 0.881           & 0.860       & 0.907        \\ \hline
\textbf{K-neighbors}  & 0.875              & 0.333           & 0.483       & 0.810        \\ \hline
\textbf{DecisionTree} & 0.805              & 0.786           & 0.795       & 0.704       
\end{tabular}}
\label{tab:ml}
\end{table}

==> OLD_IEEE/sec4_project_stats.tex <==
\begin{table}[tb]
\caption{Project statistics:NEEDS TO BE UPDATED WITH AYDA ROWS}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllll}
\textbf{Dimension}               & \textbf{Max} & \textbf{Min} & \textbf{Average} & \textbf{Median} \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Line count}              & 18,474,542   & 82,303       & 1,770,089        & 1,074,660       \\
\textbf{Duration (weeks)}        & 1,063        & 214          & 606              & 560             \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Total Developers}        & 1,852        & 21           & 226              & 106             \\
\textbf{Total Commits}           & 80,227       & 3,561        & 22688            & 18,084          \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Total Pull-request (PR)} & 32,646       & 6            & 2,692            & 589             \\
\textbf{Total PR-comments}       & 448,642      & 6            & 22,136           & 1,699          
\end{tabular}}
\label{tab:apache}
\end{table}


==> OLD_IEEE/sec4_rulebook.tex <==
\begin{table}[tbp]
\caption{Classification rule book}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll}
\multicolumn{1}{c}{\textbf{Explanation}} & \multicolumn{1}{c}{\textbf{PR-comment sample}}                                                                                                                                                                              \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Instruction}                     & \begin{tabular}[c]{@{}l@{}}"Next time please run {[}tool{]} on the project before creating a PR.\\ You would have noticed {[}problem{]}. I’ll fix it on our master."\end{tabular}                                           \\
\textbf{Suggestion}                      & \begin{tabular}[c]{@{}l@{}}"I would still duplicate {[}action{]} like I did in {[}certain PR{]} \\ because it’s widely used in the runner’s unit tests. \\ Maybe this could be removed after {[}situation{]}."\end{tabular} \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Error addressing}                & \begin{tabular}[c]{@{}l@{}}That is fine. Would you mind just doing {[}action{]} again to\\ kick off {[}framework{]}? I think{[}framework{]} is just not happy \\ when it has a lot of loads.\end{tabular}                  
\end{tabular}}
\label{tab:rulebook}
\end{table}

==> OLD_IEEE/threats.tex <==
%!TEX root = main.tex
\section{Threats to Validity}
\label{sec:threats}
\boldification{No empirical study is perfect, we have tried our best...}
Like other empirical research, our study also has threats. We taken all possible measures to offset the impact of these potential threats as we detail below.

\boldification{External validity from 1)qualitative analysis, we validate our findings from literature survey and member-checking survey. 2) We only covered PRs on Github Apache projects, but we obtained large samples }
%
External validity is identified as the capability to generalize our findings. In this study, the first threat is subjectivity of data during qualitative analysis. To reduce this threat, we validated our findings from the literature survey and by reaching out to our interviewees for member-checking. 
The second threat can arise due to our dataset comprising of pull request comments only. By considering a large sample of comments from multiple Apache projects, we mitigate bias to any particular project. 

\boldification{Internal validity from 1)objective coding for ML training, but IRR past over 90\%, 2)Namsor, not all user provides correct data, we only kept data that probability greater than 90\%}
%
Internal validity is identified as how the research design affects the study's results. 
% There are uncontrolled variables in our study.

For example, when we manually label implicit mentoring for our classifier's training dataset, the subjectivity of data can be seen as an internal validity threat. To minimize this threat, we calculated the inter-rater reliability among the two researchers, which showed a high level of agreement (94\% IRR)~\cite{}. 
%
Another threat that can arise is due to our use of the ``Namsor" API to identify gender for quantitative analysis. ``Namsor" requires a person's full name and geographic location to predict a gender. However, not all GitHub users provide this information due to privacy concerns. To mitigate this threat, we only use the predictions if the probability of prediction is greater than 90\%, as done in an earlier research study~\cite{}.





==> OLD_IEEE/todo.tex <==
All tables: 

https://docs.google.com/spreadsheets/d/1XeGK6TxAn2qQkKXU6EWvkWakiiX4F5peM6-wwIebUdE/edit#gid=459828337

\begin{itemize}
    \item Consistency check: PR-comments or PR comments
    \item consistency: contributor vs. developer
    \item difference is clear: Informal includes implicit
    \item male/female or men/women: Consistency check
    \item ALl tables should look the same...font size wise
   
\end{itemize}

Fig 2 (def, of mentoring) needs to be Table/ definition/references (otherwise doesnt look like results) 

 Table V, I dont think support is doing much. I propose remove. I wanted to highlight the Classifier we choose, but it has offset the text a bit, please fix --- Done
 
 Table II. I made some wording changes that has screwed up the width, but you can easily fix it --- Done

in method Figure, the arrows should be opp for the lenses. The lenses...point to the dataset and not the other way around --- Done

Include command in main.tex to switch between draft and final status...so, that we can easily have a clean version of the text without all the boldification/notes --- Done

Use symbol for Chi-2 --- Done

Print and and see if tables are readable....table X and others too small --- Done

MAKE the Fig 3/4 SMALL...this is VERY ANNOYING --- Done
add STD in the text--- Done
close --- Done
remove figure 4 --- Done
leave the whisker--- Done


p values--- Done

\textbf{what are the different types of the mentoring, including the formal and informal, (explicit and implicit )}

\textbf{formal and informal, within the informal there is explicit and implicit.} coffee does not 


==> Table/sec3_challenge_table.tex <==
\begin{table}[tbp]
\caption{Challenge table}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|llll}
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{000000} \textbf{}}                                                                                                                               & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{Challenge name}}}                       & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{Sample quote}}}                                                                                                                         & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Mentioned \\ by\end{tabular}}}} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{Literature}}}                                                                                                                        \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }}                                                                                           & {\color[HTML]{000000} Hard to find a mentor}                                                                     & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P1:``I always have trouble \\ getting mentors ''\end{tabular}}                                                                                                    & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P1,P2,\\P3, P5\end{tabular}}                                                     & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}\cite{steinmacher2014hard, steinmacher2015systematic}\\ \cite{trinkenreich2021women, balali2020recommending}\end{tabular}} \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Mentoring \\ in general\end{tabular}}}}} & {\color[HTML]{000000} Return on investment}                                                                      & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P2:``It's hard to assess \\ during the mentorship\\ whether the return on \\ investment is going to\\ be effective.''\end{tabular}}                                & {\color[HTML]{000000} P2,P5}                                                                                                       & {\color[HTML]{000000} \cite{silva2017long}}                                                                                                                                                  \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                                                                                                & {\color[HTML]{000000} Diverging interests}                                                                       & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P5:``Your interests tend \\ to diverge, you tend to \\ look for new mentors, \\ new areas, and new\\ people to serve.''\end{tabular}}                             & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P3,P4,\\P5\end{tabular}}                                                        & {\color[HTML]{000000} \cite{balali2018newcomers, balali2020recommending}}                                                                                                                    \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                                                                                                & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Too overwhelming to \\ navigate being \\ a mentee\end{tabular}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P4:``I really got \\ overwhelmed with \\ all the information. \\ And I didn't have \\ many ideas what to\\ ask for my mentor \\ to guide me with.''\end{tabular}} & {\color[HTML]{000000} P2,P4}                                                                                                       & {\color[HTML]{000000} \cite{balali2020recommending,  steinmacher2014hard}}                                                                                                                   \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                                                                                                & {\color[HTML]{000000} Limited resources}                                                                         & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P5:``We basically \\ had raised enough \\ funding for having \\ a full-time position.''\end{tabular}}                                                             & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P1,P2,\\P5\end{tabular}}                                                        & {\color[HTML]{000000} \cite{silva2020google}}                                                                                                                                                \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}l@{}}Formal \\ mentoring\end{tabular}}}}                          & {\color[HTML]{000000} Following through}                                                                         & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P4:``There was no \\ continuous progress of\\ mentoring, we didn't \\ know how to follow\\ up on things.''\end{tabular}}                                          & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P1,P3,\\P4\end{tabular}}                                                        & {\color[HTML]{000000} \cite{balali2020recommending, steinmacher2015social}}                                                                                                                  \\ \hline

\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}l@{}}Informal \\ mentoring\end{tabular}}}                                          & {\color[HTML]{000000} unrecognized}                                                                              & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P2:`` I leave the employee\\ doesn't have any recognition \\ for this mentorship.''\end{tabular}}                                                                 & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}P2,P3,\\P4, P5\end{tabular}}                                                    & {\color[HTML]{000000} \cite{steinmacher2021being}}                                                                                                                                          
\end{tabular}}                                                         
\label{tab:challenge}
\end{table}


==> Table/sec3_mentoring_type.tex <==
\begin{table}[!tbp]
\caption{Different flavor of mentoring}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll}
\rowcolor[HTML]{EFEFEF} 
\textbf{Mentoring} & \begin{tabular}[c]{@{}l@{}} ``A relationship between a less experienced individual,\\
called a mentee or protégé, and a more experienced\\ individual known as a mentor.''  \cite{wai2009definition}\end{tabular}                                                                                                      \\
\textbf{Informal}  & \begin{tabular}[c]{@{}l@{}} ``Informal mentoring is the natural coming together of a \\mentor and protégé.'' \cite{inzer2005review}\end{tabular}                                                                                            \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Formal}    & \begin{tabular}[c]{@{}l@{}} ``Formal mentoring relationship are those that are initiated \\ through some organizational program that assigns mentors\\ and protégé'' \cite{baugh2007formal}\end{tabular} \\
\textbf{Explicit}  & \begin{tabular}[c]{@{}l@{}} ``protégés expect and desire a relationship with a mentor who \\provides explicit direction and guidance.'' \cite{noonan2007peer}\end{tabular}                                        \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Implicit}  & \begin{tabular}[c]{@{}l@{}}Informal based relationship  between \\companies implicitly support others among daily activities.\end{tabular}                                                                                         
\end{tabular}}
\label{tab:mentoring_type}
\end{table}



==> Table/sec3_valid_table.tex <==
\begin{table}[!tbp]
\caption{Mentoring in OSS and its characteristics}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllcl}
                                                                                        &                                                                                                         & \multicolumn{3}{c}{\textbf{Provenance}}                                                                                                                                       \\ \cline{3-5} 
                                                                                        &                                                                                                         & \textbf{Interview}                 & \textbf{\begin{tabular}[c]{@{}l@{}}Member\\ Checked\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Literature\\ Survey\end{tabular}} \\ \hline
                                                                                        & \cellcolor[HTML]{EFEFEF}Suggestions                                                                     & \cellcolor[HTML]{EFEFEF}P1, P3, P5 & \cellcolor[HTML]{EFEFEF}\checkmark                              &\cite{ko2018informal, balali2018newcomers, trinkenreich2020hidden,fagerholm2014onboarding, zhou2012make} \cellcolor[HTML]{EFEFEF}                                             \\
                                                                                        & Instructions                                                                                            & P2, P3, P4, P5                     & \checkmark                                                     &\cite{ko2018informal, balali2018newcomers, trinkenreich2020hidden,fagerholm2014onboarding, zhou2012make}                                                                      \\
\textbf{\begin{tabular}[c]{@{}l@{}}Mentoring\\ Tasks\end{tabular}}   & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Mechanisms\\ to fix errors\end{tabular}              & \cellcolor[HTML]{EFEFEF}P1,P3, P5  & \cellcolor[HTML]{EFEFEF}\checkmark                              &\cite{ko2018informal, balali2018newcomers, bosu2019diversity, fagerholm2014onboarding, zhou2012make} \cellcolor[HTML]{EFEFEF}                                             \\ \hline
                                                                                        & Email                                                                                                   & P1, P3, P4, P5                     & \checkmark                                                      &\cite{balali2018newcomers, zhou2012make}                                                                      \\
                                                                                        & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Code review\\ tool (e.g \\ PR-comments)\end{tabular} & \cellcolor[HTML]{EFEFEF}P1, P3, P4 & \cellcolor[HTML]{EFEFEF}\checkmark                              &\cite{balali2018newcomers,  bosu2019diversity, fagerholm2014onboarding} \cellcolor[HTML]{EFEFEF}                                             \\
\textbf{\begin{tabular}[c]{@{}l@{}}Mentoring\\ Channels\end{tabular}} & In person/Remote                                                                                        & P4, P5                             & \checkmark                                                     &\cite{ko2018informal}
\end{tabular}}
\label{tab:val_tab}
\end{table}


==> Table/sec4_chi2square.tex <==
\begin{table}[!tbp]
\caption{$\tilde{\chi}^2$ test results of homophily preferences}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lll}
                                                                                                                & \textbf{Results}                                                                                                                                                              & \textbf{P-value (chi square )}                                     \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                        & \cellcolor[HTML]{EFEFEF}                                                                                                                                             & \cellcolor[HTML]{EFEFEF}                                   \\
\cellcolor[HTML]{EFEFEF}                                                                                        & \cellcolor[HTML]{EFEFEF}                                                                                                                                             & \cellcolor[HTML]{EFEFEF}                                   \\
\multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}l@{}}Overall\end{tabular}}} & \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}At lesat one of the group is \\ different than others in Table \ref{tab:gender_implicit}\end{tabular}} & \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\textless{}0.001} \\
                                                                                                                &                                                                                                                                                                      &                                                            \\
\multirow{-2}{*}{\textbf{Top$\rightarrow$Down}}                                                                            & \multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}At lesat one of the group is \\ different than others in Table \ref{tab:gender_implicit}\end{tabular}}                         & \multirow{-2}{*}{\textless{}0.001}                         \\
\cellcolor[HTML]{EFEFEF}                                                                                        & \cellcolor[HTML]{EFEFEF}                                                                                                                                             & \cellcolor[HTML]{EFEFEF}                                   \\
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Peer$\rightarrow$Peer}}                                                  & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}At lesat one of the group is \\ different than others in Table \ref{tab:gender_implicit}\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textless{}0.001} \\
\textbf{Bottom$\rightarrow$Up}                                                                                         & \begin{tabular}[c]{@{}l@{}}At lesat one of the group is \\ different than others in Table \ref{tab:gender_implicit}\end{tabular}                                           & $<0.001$                                          
\end{tabular}}
\label{tab:chi2}
\end{table}

==> Table/sec4_homophily_Z.tex <==
\begin{table}[tbp]
\caption{Proportion test results of homophily preferences }
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllll}
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{000000} \textbf{}}                                         & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{Overall}}} & \textbf{Top$\rightarrow$Down} & \textbf{Peer$\rightarrow$Peer} & \textbf{Bottom$\rightarrow$Up} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Z-score}                                                         & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}202.22}                                  & 145.86                        & 120.90                         & 70.77                         \\
\rowcolor[HTML]{FFFFFF} 
\textbf{P-value}                                                         & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}$<$ 0.001}                               & $<$ 0.001                     & $<$ 0.001                      & $<$ 0.001                      \\
\rowcolor[HTML]{EFEFEF} 
\textbf{\begin{tabular}[c]{@{}l@{}}Estimated\\ differences\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}0.88}                                    & 0.88                          & 0.86                          & 0.90                          \\
\rowcolor[HTML]{FFFFFF} 
\textbf{Cohen d}                                                         & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}2.13}                                    & 2.16                         & 2.07                           & 2.25                           \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{l}{\cellcolor[HTML]{EFEFEF}$H_0: P_1-P_2 = 0$, $H_a: P_1-P_2 \neq 0$, adjusted $\alpha=0.017$}                                                                                                                                                                            \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{5}{l}{\cellcolor[HTML]{FFFFFF}$P_1$: (m$\rightarrow$m + w$\rightarrow$w) / All mentoring PR-comment}                                                                                                                                                 \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{l}{\cellcolor[HTML]{EFEFEF}$P_2$: (m$\rightarrow$w + w$\rightarrow$m) / All mentoring PR-comment}                                                                                                                                                
\end{tabular}}
\label{tab:sec4_homophily_Z}
\end{table}


==> Table/sec4_homophily_gender_diff-OLD.tex <==
\begin{table}[!t]
\caption{Proportion test results of homophily preferences for each gender}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllll}
                                                                                 & \textbf{Overall}   & \textbf{Top$\rightarrow$Down}   & \textbf{Peer$\rightarrow$Peer}  & \textbf{Bottom$\rightarrow$Up}  \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Proportion Z-test}                                                       & P1 $\neq$ P2       & P1 $\neq$ P2           & P1 $\neq$ P2             & P1 $\neq$ P2        \\
\textbf{P-value}                                                                 & \textless{}0.001   & \textless{}0.001       & \textless{}0.001         & \textless{}0.001    \\
\rowcolor[HTML]{EFEFEF} 
\textbf{\begin{tabular}[c]{@{}l@{}}Estimated ratio\\ differences\end{tabular}}   & 0.454              & 0.807                  & 0.086                    & 0.846               \\
\textbf{Effect size}                                                             & 1.243              & 1.946                  & 0.493                    & 2.048               \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{l}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}
%NEW: P1:Proportion of homophily mentoring of men (m$\rightarrow$m/ (m$\rightarrow$w + m$\rightarrow$m))\\ 
%NEW:P2:Proportion of homophily mentoring of women men (w$\rightarrow$w/ (w$\rightarrow$m + w$\rightarrow$w)\end{tabular}}

OLD: P1:Proportion of homophily mentoring of men (m$\rightarrow$m/ (m$\rightarrow$w + m$\rightarrow$m + w$\rightarrow$m))\\ 
OLD: P2:Proportion of homophily mentoring of women men (w$\rightarrow$w/ (w$\rightarrow$m + w$\rightarrow$w + m$\rightarrow$w)\end{tabular}}
\end{tabular}}
\label{tab:pro_gender_samegender_OLD}
\end{table}






==> Table/sec4_homophily_gender_diff.tex <==
\begin{table}[!t]
\caption{Proportion test results of homophily preferences for each gender}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllll}
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{000000} \textbf{}}                                         & {\color[HTML]{000000} \textbf{Overall}} & {\color[HTML]{000000} \textbf{Top$\rightarrow$Down}} & {\color[HTML]{000000} \textbf{Peer$\rightarrow$Peer}} & \textbf{Bottom$\rightarrow$Up} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Z-score}                                                         & 61.97                                   & 52.31                                                & 16.92                                                 & 60.82                          \\
\rowcolor[HTML]{FFFFFF} 
\textbf{P-value}                                                         & \textless0.001            & \textless0.001                         & \textless0.001                          & \textless0.001   \\
\rowcolor[HTML]{EFEFEF} 
\textbf{\begin{tabular}[c]{@{}l@{}}Estimated\\ differences\end{tabular}} & -0.16                                   & -0.44                                                & -0.02                                                 & -0.750                         \\
\rowcolor[HTML]{FFFFFF} 
\textbf{Cohen d}                                                         & 0.62                                    & 1.16                                                 & 0.21                                                  & 0.33                           \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{l}{\cellcolor[HTML]{EFEFEF}$H_0: P_1-P_2 = 0$, $H_a: P_1-P_2 \neq 0$}                                                                                                                                                                              \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{5}{l}{\cellcolor[HTML]{FFFFFF}$P_1$: m$\rightarrow$m/ (m$\rightarrow$w + m$\rightarrow$m)}                                                                                                                                                             \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{5}{l}{\cellcolor[HTML]{EFEFEF}$P_2$: w$\rightarrow$w/ (w$\rightarrow$m + w$\rightarrow$w)}                                                                                                                                                            
\end{tabular}}
\label{tab:pro_gender_samegender}
\end{table}





==> attic/define.tex <==
\section{Mentoring Approaches in OSS}
\label{sec:3}
In this section, we report on the different approaches to mentoring in OSS projects. OSS projects and foundations have invested in different mentorship programs such as, the Google Summer of Code by the Apache Software Foundation that paired 1,289 student with mentors from across OSS organizations in summer of 2021\cite{googlecode}. The Linux foundation currently has 7 mentorship programs and has invested over 2.5M USD in support of first-time and underrepresented OSS contributors~\cite{linux}. 

However, outside of such formal mentorship programs, contributors actively seek guidance and support from each other via informal venues such as direct contact or meeting at conferences. Moreover, technical guidance is also provided when contributors review code. Currently, not much is known about the different flavors of mentoring taking place in OSS. Without an understanding of the different types of informal mentoring taking place in OSS, it would be difficult to acknowledge the important contributions made by OSS mentors. We close this gap by investigating the different flavors of mentoring in RQ$\#1$.  


\subsection{Methodology}
As a formative study to identify the different approaches to mentoring we used semi-structured interviews along with member checking and a literature review of mentoring in the context of OSS, as shown in Figure~\ref{fig:method} A.

\begin{figure*}[!tbp]
\centering
\includegraphics[width=7in]{pic/method_vertical.png}
\caption{Overview of research method: (A) presents the formative study method used to define implicit mentoring (Section~\ref{sec:3}), and (B) presents the method used to identify and characterize implicit mentoring in a subset of OSS projects (Section~\ref{sec:4}).}
\label{fig:method}
\end{figure*}


\subsubsection{Formative Interviews}
We first conducted semi-structured interviews with five OSS developers to learn of their experiences regarding mentoring---both from the perspective of being a mentor and a mentee. \input{Table/sec3_participant_demo}
We recruited two developers, one from the Apache Source Foundation and another from the Linux Foundation, both of whom have spearheaded mentoring programs in OSS. We then used snowballing sampling method to recruit three additional participants. We stopped after five interviews, since we had already reached saturation---participants responses were similar regarding the different types of mentoring they had seen.

The interviews were done remotely, lasting around 30 minutes each. 
Each interview was recorded with participants' consent (following university-approved IRB protocol) and transcribed. 
Participants were offered a \$50 gift card as compensation for their time.
Table \ref{tab:participant_demo} presents the demographic information of our participants.

\boldification{At the beginning of the interview, we have explained our goals, and we asked participants about their mentoring experiences including formal and informal}
We briefly explained the goal of the interview to the participants in the beginning of the interview. We asked participants about their roles and experiences in OSS, their mentoring experiences including formal and informal, what they consider to be informal mentoring and their opinions regarding formal and informal mentoring in OSS. At the end of our interview, we asked participants on how mentoring can be improved in OSS. See \hl{companion website}~\cite{} for interview questions. 

\boldification{We transcribed the interview recordings and we used negotiated agreement to reached a consensus on the code category and rule set}
We transcribed the interview recordings and qualitatively analyzed the transcripts, following open coding protocol---an analytic process by which concepts (codes about mentoring) that are the observed in the interview data are attached during the data analysis. 
followed the principles of grounded theory to code for types of mentoring, challenges of mentoring and implicit mentoring. 
Two researchers performed the analysis by independently coding all the transcripts creating codes regarding types of mentoring and challenges, how and where  mentoring was provided, and recommendations. During this analysis, each emerging code was compared with the existent codes to determine if the emerging code was a discrete category or a subset of an existing code. After this step, the two researchers met to discuss their codes and performed card sorting to arrive at the final code set~\cite{izquierdo2021long}.
% During this step, researchers constantly compared the emerging codes with the by comparing with existing codes. After this step, the two researchers met to discuss their codes and reach negotiated agreement \cite{izquierdo2021long}.
%

\subsubsection{Validating findings from past literature and member checking}

\boldification{To understand what constitutes mentoring and the different flavors of mentoring research in the field of OSS mentoring}

%To understand what constitutes mentoring and the different flavors of mentoring research in the field of OSS mentoring, we conducted a literature survey. To do that, we searched for the keywords: "mentoring", "formal mentoring", "Informal mentoring". We chose papers which were published in top conferences from 2012 to 2021 such as IEEE-ICSME, IEEE-RSSE, IEEE-ICGSEW, ACM-FSE, ACM-ESEM, ACM-ICSE, IEEE-ICSME, IEEE-MSR, ACM-SIGCSE, ACM-HCI, and ACM-ICPS. Then, the first author read the titles and abstracts and only selected those which talked about mentoring in the abstract, to find the relevant papers. This step resulted in 23 papers.
We validated the insights from our analysis in two ways: member checking and a literature review.

\boldification{In addition to the literature survey, we continue validating our findings through member checking survey.}
\textit{Member Checking}: We validated our findings by via member checking with our interview participants.
We contacted each of our participants through email and sent them a survey that comprised 15 questions and was conducted via Qualtrics (see \hl{companion website}~\cite{} for survey questions). The survey included demographics questions (4), questions about what constitutes mentoring and where it occurs (3), and a sample of Pull-Request comments (8). 

All questions had associated text boxes for participants to provide additional feedback. The eight pull requests were randomly selected from our dataset based on their verbosity and participants were asked to ascertain if the comment was mentoring (or not) and provide a rationale for their decision. The open ended responses were used to refine our understanding of the different approaches mentoring and the code set.

\textit{Literature review}:
To corroborate our findings from the interviews, we conducted a small-scale systematic mapping study. 
According to Kitchenham et al.~\cite{kitchenham2015evidence}, the goal of such a mapping study is to survey the available knowledge about a topic. To determine the optimal set of search keywords, we first conducted a pilot search on two well-known digital libraries---IEEE and ACM. 
This process helped us identify relevant words used in mentoring literature in Software Engineering, especially in OSS. Our final list of search keywords included : {``mentor'', ``mentoring'', ``formal'', ``Informal''}.

Next, to discover relevant publications for the survey, we used three of the most popular online paper search engines: ACM Digital Library, IEEE Xplore, and Scopus and searched for papers that were published in top conferences from 2012 to 2021 such as, IEEE-ICSME, IEEE-RSSE, IEEE-ICGSEW, ACM-FSE, ACM-ESEM, ACM-ICSE, IEEE-ICSME, IEEE-MSR, ACM-SIGCSE, ACM-HCI, and ACM-ICPS. Our initial search resulted in 54 publications. Then, the first and second author read the titles and abstracts and only selected those which talked about mentoring in the abstract, which resulted in 17 papers. 
%To narrow down the search results, next, we filtered out publications that were not part of our inclusion criteria. 
Our search criteria may have resulted in leaving out some relevant studies. 
Thus, we conducted backward snowballing~\cite{wohlin2014guidelines} (\textit{i.e.,} looking for additional studies in the reference lists of the selected studies, 
as suggested by Keele et al.~\cite{keele2007guidelines}). We performed a single iteration of backward snowballing, which provided 6 additional papers. Our final list consisted of 23 papers.


\subsection{Results:} 
Mentoring is an important part of onboarding and career progress in OSS [??]. However, despite formal programs, it is hard for mentees to find mentors: ``\textit{I always have trouble getting mentors...}'' [P1], \cite{steinmacher2014hard, steinmacher2015systematic, trinkenreich2021women, balali2020recommending}. On the flip side, it is hard for mentors to make a commitment without knowing whether their effort would be worthwhile:``\textit{It's hard to assess...whether the return on investment is going to be effective}.'' [P2], \cite{silva2017long}

There are two dimensions to mentoring. The first is whether the mentorship is Formal or Informal. The second is whether mentoring is Explicit or Implicit. 

\textit{\textbf{Formal mentoring}} includes programs where mentors and mentees are formally connected through either through scholarships or mentoring programs~\cite{balali2018newcomers, balali2020recommending}. However, despite the formal programs having guidance and financial support, it is difficult for mentees to figure out how to seek guidance: ``\textit{I really got overwhelmed with all the information...I didn't have much idea what to ask for my mentor to guide me with}''[P4] \cite{balali2020recommending, steinmacher2014hard},
and follow up with their mentors: ``\textit{There was no continuous progress of
mentoring, we didn't know how to follow
up on things}''[P4], \cite{balali2020recommending, steinmacher2015social}.
%
Sustaining the mentor-mentee relationship was further difficult because of (a) diverging interests: ``\textit{...interests tend to diverge, you tend
to look for new mentors, new areas, and new people to serve.}''[P5], \cite{balali2018newcomers, balali2020recommending} and (b) limited resources: ``\textit{We basically had to raise enough funding
for having a full-time position}.''[P5], \cite{silva2020google}.


%
%\input{Table/sec3_challenge_table}
% As our interview participant P2 mentioned ``It's hard to assess during the mentorship.''
% Overall, out interviews identified seven challenges of mentoring in OSS, as shown in Table~\ref{tab:challenge}. 
% A lot of research (Table~\ref{tab:challenge}) as well as organizations have put in work to create formal mentorship programs, but these have specific challenges as our interviewees reported.

%\end{comment}
\boldification{Informal mentoring is more effective than formal mentoring. }
%
\textit{\textbf{Informal mentoring}}, perhaps because of the above challenges, can be more effective than formal mentoring~\cite{inzer2005review}. Informal mentoring is ``interest driven" when a mentor or mentee reaches out to the other to seek/give guidance in a particular area. Informal mentoring occurs frequently: ``\textit{I have always had mentors, all informal mentors, because I chose to learn from them}''[P1],~\cite{inzer2005review, okurame2005role, ko2018informal}. 
Informal mentoring can be explicit, where the mentee or mentor reaches out to the other or can be implicit (discussed next).
In either case, such mentoring is ``invisible" and the effort made by mentors remain unacknowledged: ``\textit{``I believe the employee doesn't have any recognition for [informal] mentorship.}'' [P1], \cite{steinmacher2021being}.


% Inzer and Crawford \cite{inzer2005review} stated that informal mentoring is more effective than formal mentoring. People regularly go and find informal mentors because of the effectiveness. Unlike formal mentoring, informal mentoring can happens at anytime \cite{ko2018informal}.Our participants stated that ``I have always had mentors, all informal mentors, because I chose to learn from them'' (P1); ``Informal is mostly how I do it all these days'' (P5);  ``I think informal mentoring, it's something that I really enjoy'' (P4), which are inline with these papers \cite{inzer2005review, okurame2005role, ko2018informal}.

Both the formal and informal approaches that has been investigated in literature are explicit, where mentees seek out or are formally paired with mentors. However, mentoring need not always be explicit and can be done in a developers' every day activities, such as code review: ``\textit{When somebody reviews a patch, that gives a feedback to you, that's a form of mentoring}''[P1]. 

\textit{\textbf{Implicit mentoring}} can be defined as mentoring that occurs in everyday development activities such as code reviews, where a mentor provides an underlying explanation when providing suggestions, instructions, or mechanism to address errors. Such mentoring can be through multiple channels: email, pull request comments, or even through meetings help in person or through online communication tools. As P3 commented ``\textit{There's going to be mentors who are more like code reviewers or the design reviewers...mentorship that happens every single day''}.

Table~\ref{tab:val_tab} presents the different types of mentoring guidance given across the different channels in OSS, which we identified from the interivews, as well as corroborated by liteature on mentoring. It also lists where and how often such mentoring occurs.


%\input{Table/sec3_mentoring_type}
%And P3 said: ``There's going to be mentors who are more like code reviewers or the design reviewers.''

%while it actually happens a lot [shuah quote], diverging interests (a problem with formal) is not a problem [kate; quote], is important for the project/contribution to be on track [Steve to find quotes], not limited to seniority (P3 "seniority is not important for informal mentoring."), does take time [quote...]


%
\input{Table/sec3_valid_table}
% Unfortunately, implicit mentoring is not well recognized:
% P1: ``I believe the employee doesn't have any recognition for [informal] mentorship.''
% P3: ``No, I don't think the mentorship is recognized at all in the foundation.''
% In the next section we fill this gap by automatically identifying implicit mentoring within PR comments.

%Story0:
%Mentoring is much needed, when successful, its awesome, but there are several challenges that exist [...]. Our interviews identified these x challenges ["challenges table" ]

%A lot of work in lit as well as regular OSS is put in creating formal mentorship programs, but these have specific challenges our interviews talked about [point to "challenges table"].

%People regularly go and find informal mentors. Although, effortful, many people do that. Quote , which is inline with these papers [paper references].

%...but these have these challenges [ref "challenges table"]

%However, there is another type of informal mentoring that happens in OSS which is implicit in the day to day activities. [Quote]:

%Therefore, mentoring can be seen as these set of activities (figure1: "diff flavors"). 

%here, we explore implicit mentoring deeper, because....while it actually happens a lot [shuah quote], diverging interests (a problem with formal) is not a problem [kate; quote], is important for the project/contribution to be on track [Steve to find quotes], not limited to seniority [], does take time [quote...].

%Implicit mentoring definition:

%Implicit mentoring involves these types of stuff:
%[validation table for Imp. Mentoring definition]

%Implicit mentoring happens in these channels
%[validation table 1 for channels]

%Unfortunately, implicit mentoring is not well recognized: Quote....so, in next section we fill this gap by automatically identifying

%STORY:1

%Formal mentoring has challenges, the satisfaction is missing from both mentor and mentee
%SO....what do I do with this....Why care: not all OSS devs have chance to get formal mentoring...so why try to investigate...how people are getting mentored outside of formal mentoring programs


%Definition/hierarchy of Mentoring- formal/informal (explicit, implicit)


%Informal...explicit is hard to recognize [due to channel == outside of work...]
%SO, why should I care/what do I do

%Channels of implicit mentoring in these communication tools...seems recognizable
%Implicit mentoring definition:giving suggestions/instructions/addressing errors bugs etc.
%So, what do I do with this

%Story2
%There are various mentoring programs for newcomers in OSS. However, they are not very helpful In OSS, developers often get mentored informally. In two ways: Explicitly, by reaching out to people and implicitly, on pull request channels during code reviews and discussions on submitted PRs. Explicit mentoring is hard to identify since they do not happen over public channels. However, implicit mentoring happens very frequently in daily activities on the public communication channels and the developers doing the mentoring go unnoticed and are not acknowledged. We want to understand to what extent implicit mentoring is happening in day-to-day tasks. 


%
%Analysis from qualitative analysis, we observe that the mentoring in OSS has two majority types: formal and informal mentoring. 
%
%As for informal mentoring, Inzer and Crawford state "a relationship between two people where one gains insight, knowledge, wisdom, friendship, and support from the other", which is same in OSS community  \cite{inzer2005review}.
%
%\textbf{However, mentoring is necessary for all developers and organizations, Table indicates that mentoring is happening everyday, it is necessary to find a mentoring system for all developers and organizations.}
%
%However, mentoring is necessary. Software developers needs to learn everyday. P4: "Considering yourself somebody always learning, always, you're always learning more." And the Table \ref{tab:inter} indicate the frequency of the mentoring of each member. 
%
%Thus, it is extremely important to have a appropriate mentoring system for developer in OSS, not just new comers, but for all developers and organizations. 





%\begin{table}[thp]
%\begin{tabular}{|l|l|}
%\hline
%\multicolumn{1}{|c|}{\textbf{Categories}} & \textbf{References} \\ \hline
%"giving instructions"                       & \cite{balali2020recommending}  \cite{steinmacher2012recommending} \cite{fagerholm2014onboarding}                \\ \hline
%"overcoming barriers"                       & \cite{balali2020recommending} \cite{hsieh2013welcome} \cite{fagerholm2014role}                    \\ \hline
%"supporting developments"                   & \cite{hsieh2013welcome} \cite{hsieh2013welcome} \cite{berlin1993beyond} \cite{fagerholm2014role}                    \\ \hline
%"Providing suggestions"                     & \cite{balali2020recommending} \cite{steinmacher2012recommending}                   \\ \hline
%\end{tabular}
%\label{tab:t1}
%\end{table}



















==> attic/identify.tex <==
\section{Implicit mentoring and its characteristics}


\label{sec:4}

\boldification{we answer RQ2 by focusing on PR-comments because...}
In this section, we report on how to identify and characterize implicit mentoring in OSS projects (RQ \#2). Our goal here is to investigate how to automate the identification of implicit mentoring taking place on an everyday basis, but remaining unacknowledged.
Here we focus on implicit mentoring occurring via PR-comments as it a prominent channel via which developers provide feedback and mentoring as found by Kononenko et al.~\cite{kononenko2018studying} and mentioned by our interview participants (cf. Section~\ref{sec:3}). 


\boldification{past work shows mentoring to be dyadic, topc-down, we investigate this}
Traditionally, mentoring has been viewed as a dyadic relationship wherein an experienced individual (the mentor) provides practical advice and guidance to an inexperienced individual (the mentee)~\cite{Kram_1988, gandhi2012reverse}, helping them gain technical and job-related skills~\cite{brashear2006exploratory, hale2000match}. Therefore, we wanted to analyze if the same sort of mentoring dynamics occur in implicit mentoring, leading to:\\
\textit{RQ2a: To what extent is implicit mentoring characterized by dyadic, top-down interactions?}. 


\boldification{past work has shown women do more mentoring, low gender numbers, and homophily, so we investigate this}
Additionally, past work has found that women, especially in OSS, are more tuned to community building roles~\cite{??} and end up being mentors more often~\cite{??}. This often translates to women seen as community managers and losing their ``engineer'' voice in decision making~\cite{??}. Further, given the gender imbalance in OSS (past work having found women contributors to range around 10\% ~\cite{}) and past research having shown that same-gender mentor-mentee dyadic relationships are more common~\cite{}, it can mean that fewer women have mentors. Both of these phenomena disadvantage women in OSS. Therefore, we wanted to investigate if they also occur in implicit mentoring, leading to:\\
\textit{RQ2b: What role do women play in implicit mentoring?}


\subsection{Method}


\boldification{we chose Apache and these projects because...}
Figure \ref{fig:method} B presents the overview of our methods.
\textbf{Project Selection}: We use a set of 37 Apache projects as our data corpus to answer RQ\#2. We selected Apache projects since one of the most mature OSS ecosystems with well defined policies and a philosophy of transparency where all discussions should be conducted in online forums, which is essential for us as we aim to extract implicit mentoring from archived communication. Further, the Apache Source Foundation is committed to facilitating and improving mentoring in OSS. In addition to providing explicit guidelines for mentors~\cite{???}, it also oversees one of the most popular formal mentorship programs (The the Google Summer of Code~\cite{??}), which would mean that the philosophy of mentoring is instilled in Apache contributors.  Finally, Apache projects are often studied in scientific research, which allows our work to be placed in the context of existing research~\cite{gharehyazie2015developer,kabinna2016logging,chen2017characterizing,chelkowski2016inequalities,oliva2015evolving}. In fact, we reuse the dataset curated by Mannan et al.~\cite{mannan2020relationship}


\boldification{Our dataset contained this 97,444 PRs and this 588,094 PR-comments across these 11,634 authors.}
Table \ref{tab:apache} presents the statistics of the 37 projects in our dataset. The criteria for selecting the dataset was that projects are mature and include sizeable codebase and contributors (which are satisfied by the Mannan et al. dataset). In total, our dataset comprises 97,444 pull-requests, 588,094 PR-comments logged by 11,634 (unique) PR-comment authors. See Supplemental~\cite{Link} for further details about each project in the dataset.
\input{Table/sec4_project_stats}


\boldification{we manually classified implicit mentoring this way and did IRR}
\textit{\textbf{Manual Classification of Sample Data}}: 
To answer our research questions, we need to first differentiate between PR-comments with/without implicit mentoring. As manual classification is not a practical option to classify $588,094$ PR-comments, we use machine learning techniques. To train the machine learning algorithm we needed to manually classify a training set.  
We determine the size of the training dataset by using a 95\% confidence interval and a margin of error of 5\% \cite{kotrlik2001organizational} on the dataset, giving us a sample size of 384 PR-comments.
We then randomly selected the 384 PR-comments from the full dataset to manually classify all its associated comments.


Next, the first two authors manually labeled a subset of the PR-comments in the training set with binary labels based on whether the PR-comment included implicit mentoring to calculate Inter Rater Reliability (IRR) \cite{hallgren2012computing}. A PR-comment was considered to contain implicit mentoring, if it included an ``explanation''in addition to giving suggestions, instructions or helping fix errors (see ~\ref{sec:3}). Table~\ref{tab:rulebook} shows the rule book we used with examples of PR-comments. 
\input{Table/sec4_rulebook}


The two authors independently labeled 20\% of the PR-comments independently and reached high IRR (94\% Cohen Kappa~\cite{viera2005understanding}).The remaining 80\% of the training dataset was split evenly between the two authors who manually classified the PR-comments. 
%


\textit{\textbf{Machine Learning Classifier}}:

Using the manually classified corpus, we train four different machine learning classifiers, aRandom Forest \cite{pal2005random}, a Bernoulli \cite{singh2019comparison}, a Support Vector \cite{cortes1995support}, a KNeighbors \cite{laaksonen1996classification}, and a Decision trees \cite{kothari2001decision}. 

\boldification{Table presents the machine learning classifier comparison results. After comparison, we chose the random forest classifier.}
\input{Table/sec4_ml_results}
%\as{we need to give more details about hyper-parameter optimization}
%\zf{methods are shown in comments}
Table~\ref{tab:ml} shows the precision, recall, F1, and AUC scores of all the classifiers we implemented. 
We used RFC because it had the best overall performance among the five classifiers we implemented. SVM and RFC had similar AUC scores. However, identifying some false positives as mentoring is better than having more false negatives, since we want to minimize undiscovered implicit mentoring instances. Before we select the best performance classifier. To ensure the best performance, we applied hyper-parameter adjustments \cite{horvath2016effects} from Python Scikit learn library \cite{pedregosa2011scikit} to all five classifiers. Randomized look sets up a lattice of hyper-parameter values and chooses arbitrary combinations to train each classifier. By applying $Scikit-Learn RandomizedSearchCV$, we found the optimal parameter for each classifier.Our hyper-parameter grid for the best classifier (Random forester) includes $n_estimators$, $max_features$, $max_depth$, $min_samples_split$, $min_samples_leaf$, and $bootstrap$. The final tuned Random forester parameters for our classifier were $n_estimators = 600$, $max_features = auto$, $max_depth = 90$, $min_samples_split = 5$, $min_samples_leaf = 2$, and $bootstrap = True$.  The model was trained with 80\% data sample and tested with 20\% data sample. Thus, we chose the classifier with a greater recall, that is, RFC.
%AYDA TEXT: We performed hyper-parameter optimization using randomized search~\cite{bergstra2012random} for all four classifiers before selecting the decision tree. Randomized search sets up a grid of hyper-parameter values and selects random combinations to train the model and score on the validation data. The number of search iterations is set based on time/resources; in our case, it was 10. We search for the optimal parameter settings using the Scikit-Learn RandomizedSearchCV function. Our hyper-parameter grid for the best classifier (Decision Tree) includes ``max\_depth'',``max\_features'', ``min\_samples leaf'' and ``criterion''. The final tuned decision tree parameters for our classifier were ``min\_samples\_leaf: 5, max\_depth:3, max\_features: 5, criterion: gini''.


\boldification{We need to identify mentors/mentee and their seniority  to answer RQ2a. We identify mentee/mentors this way}
\textit{\textbf{Identifying Expertise of Mentors and Mentees}}: 
In order to investigate the extent to which top-down interactions comprise implicit mentoring (RQ2a), we need to first identify when someone is a mentee or a mentor and their experiences. We considered the PR author as a mentee if any of the PR-comments associated with that PR is classifed as ``mentoring''. Note that, PRs that received no PR-comments and were directly accepted or rejected are not included in this analysis. For those PR-comments that are identified as mentoring, their authors are identified as a mentor.


\boldification{we use project/GH exp as a proxy for seniority. We calculate experience this way} 
To investigate the dynamics of implicit mentoring, especially if it comprises top-down interactions (experienced to inexperienced) we calculate experience at two levels. First, experience within the specific project, which we calculated based on the date of their first commit in that project by doing this \as{add me}. However, in OSS, contributors can participate in multiple projects or can leave a project to join another. In such cases, they may bring experiences in working on another project when mentoring a developer in a project. Therefore, we also calculate the overall experience of a mentor in GitHub based on the first commit \as{this way...add me}. Note, that when analyzing the experience of mentors in GitHub, there were cases where the developers had set their profile settings to ``private'' or never committed on any repositories, such as automated replying ``bot'' users. There were 413 such profiles (3.43\% of PR-comment authors). To enable a systematic investigation of project-specific and overall experiences, we removed these developers from this analysis in RQ2a.  


\textit{\textbf{Identifying Gender}}: 
\boldification{To investigate the gender diversity of implicit mentoring in OSS, we first mined the information of each mentor we have identified. We applied ``Namsor'' tool to identify the mentor's gender based on the geographic information.}
We also explored the gender dimension of participants to answer RQ2. We know that women are a minority in OSS community \cite{canedo2020work}. Previous research found that mentor relationships involving homogenous or diverse relationships involving female mentors provide more role demonstrations and less professional development than relationships involving male mentors. Homophily man mentoring relationships provided less psychosocial support than woman homophily women relationship \cite{sosik2000role}. Therefore, investigating the gender diversity of OSS implicit mentoring would help the OSS community to understand the effectiveness of mentoring relationship regarding genders. We used the ``Namsor'' API to identify their gender based on their full name and geographic information we retrieved from GitHub API. ``NamSor'' is a name recognition API that estimates the gender of a name on a -1 to +1 probability scale based on geographic information. \cite{namsor}. Multiple studies have addressed the reliability of the ``Namsor'' gender classifications, the error is less than 10\%\cite{santamaria2018comparison, santamaria2018comparison}. Note that not all users had provided their full names and geographic location on GitHub. Thus, after applying the ``Namsor'' API, we used the results to do further analysis only if the identified gender probability is over 90\%.


\boldification{we used statistical tests to analyze the gender dimension for implicit mentoring from three aspects: proportions, homophily, and cross gender mentoring}
%In addition, we used statistical tests to analyze the gender dimension for implicit mentoring from three aspects: comparison between proportions implicit mentoring given by men and women; comparison of homophily preferences of implicit mentoring between men and women; and comparison of cross-gender mentoring given by men with women. 
It is known that women developers are significantly less than men developers in OSS \cite{canedo2020work}. In this study, we continue exam the effect of gender composition for implicit mentoring. We first wanted to exam the proportion of mentoring given by men and women by two sample Z-test of proportions \cite{ld1993biostatistics}. Compared with homophily mentoring, cross-gender mentees are less likely to participate in activities after formal mentoring sessions \cite{ragins1990perceptions}. Since implicit mentoring is part of informal mentoring, we continued to examine the homophily preferences of implicit mentoring in OSS by conducting a two sample Z-test of proportions. What is more, previous studies on other domains examined the effect of gender during mentoring and conclude that men are doing more homophily mentoring than women \cite{ragins1999mentor}. To expand the homophily studies of implicit mentoring of each gender, we therefore, tested the proportion of cross-gender mentoring of each gender. In addition, for each of the test mentioned above, we performed exact test for different experience mentoring approaches simultaneously. To reduce the false-positive results for experiences mentoring approaches, we applied Bonferroni correction to adjust $P$ values \cite{napierala2012bonferroni}. 


\subsection{Results}
Here we first discuss to what extent implicit mentoring occurs in our dataset and then characterize it through the type of mentoring interactions ($RQ \#2a$) and gender ($RQ \#2a$) lenses. 

\boldification{overall numbers show implicit mentoring is pervasive}
As a first step, we investigate how often implicit mentoring occurs via PR-comments. Our results show that a majority of PRs included implicit mentoring (67.53\% out of 974,44 PRs). A single PR can have multiple rounds of discussion between the PR-author and other developers, which is recorded via the PR-comments. In our dataset on an average a PR had 6.035 comments ($sd=8.054$). It is then possible that one or multiple of these comments could embed implicit mentoring. In our dataset a large portion of PR-comments embedded implicit mentoring (31.00 \%) and a majority of the developers provided such mentoring (70.73\% out of 11,634 developers). This shows that implicit mentoring is quite pervasive. Next, we characterize implicit mentoring further.


\subsubsection{Interaction Types in Implicit Mentoring (RQ \#2a)}
\label{flavors}

\begin{figure}[!tbp]
\centering
\includegraphics[width=3.5in]{pic/pr_mentoring.png}
\caption{Number of instances of implicit mentoring PR-comments vs. difference in experiences of mentor/mentee}
\label{fig:PR}
\end{figure}


\boldification{Surprisingly...peer mentoring is the most common mentoring approach from our observations, within identified 67.583\% PRs contain implicit mentor, dyad (62.06\%): 40,837, triad (23.68\%): 15,585, >triad(14.26\%):9,383 }
%
Here we investigate to what extent implicit mentoring includes dyadic, top-down interactions ($RQ \#2a$).

We answer the first part of the question by considering the interactions for each PR. The PR-author is considered the mentee. Authors of PR-comments that included implicit mentoring are considered mentors. If the discussions occurred only between the mentee and one mentor, this mentoring is considered \textit{dyadic}. Similarly, if the discussions occur between an author and two mentors, its considered a triad. Finally, we group all mentee-mentor groups equal to or greater than four as $\ge$quadrad. Note, that for a PR, if there were other authors who commented, but were not mentors (comment was not considered mentoring), they are ignored in this analysis. 

Of the 65,805 PRs with implicit mentoring the majority was dyadic (62.06\%), lining up with the traditional view of mentor-mentee relationship. However, because of the open, voluntary-based  nature of OSS we found 23.68\% of mentoring occurring in triads and another 14.26\% in $\ge$quadrads. This is akin to ``it takes a village...'' adage, where the community of developers work together to mentor developers and providing perhaps different perspectives and guidance. 

\vspace{0.3cm}
\begin{mdframed}[roundcorner=10pt]
\textbf{Observation 1:} A majority of implicit mentoring is dyadic (62.6\%), but in a substantial number of cases (24,968 instances) multiple mentors provide support. \end{mdframed}
\vspace{0.3cm}

Next, we investigate what role experience---within the project and overall---plays in implicit mentoring. There can be three types of mentoring directionality:

\begin{itemize}
    \item \textit{top-down}, the mentor is more experienced than the mentee,
    \item \textit{peer-to-peer}, the mentor and mentee have same level of experience,
    \item \textit{bottom-up}, mentee is more experienced than the mentor.
\end{itemize}


To obtain the direction of mentoring, we subtracted the first commit date of the mentee from that of the mentor. If the the difference is positive, then the PR-comment interaction is flagged as \textit{top-down} and if negative it is \textit{bottom-up}. If mentor and mentee had their first commits on the same day, then it is \textit{peer-to-peer}. 


Figure \ref{fig:PR} shows the distribution of these types of implicit mentoring when considering within the project (based on the first commit in the project, marked in blue) as well as overall experience, where we use the first commit by an author in GitHub as a proxy (yellow). 


About 31\% of implicit mentoring falls in the traditional top-down mentoring interaction style. The average difference between mentee and mentor experience was 608 days ($sd=567$). 10\% of implicit mentoring where in the bottom-up category with the mean difference between mentor-mentee being 361 days ($sd=444$).
The majority was in the peer-to-peer mentoring group---59\% accounting for 182,532 mentoring instances. 


One reason for this contradiction to the traditional view of top-down mentoring could be because in OSS, developers frequently contribute to multiple projects or migrate across projects~\cite{onion paper}. In such cases, they may accrue skills and experiences relevant to the project elsewhere. Therefore, we look at the mentoring directionality when considering the overall experience in GitHub. The results of this analysis was very similar to the within-project experience analysis, with the majority of implicit mentoring instances being peer-to-peer (59\%).
This was followed by \textit{top-down} mentoring (25\% of cases with mean difference in experience being 988 days ($sd=740$)) and \textit{bottom up} mentoring (16\%, mean difference being 842 days ($sd=676$)).


When looking from the perspective of the developers who do mentoring, the story remains the same, with about 90\% of developers in our dataset having done peer-to-peer mentoring. 
This shows that “\textit{seniority is not necessary for implicit mentoring}” [P3]. 


\vspace{0.3cm}
\begin{mdframed}[roundcorner=10pt]
\textbf{Observation 2:} Peer-to-peer mentoring is the most common form of implicit mentoring accounting for 59\% of cases, followed by top-down and bottom-up flavors of mentoring.
\end{mdframed} 
\vspace{0.3cm}


\boldification{We identify gender through Namesor and tabel shows the distribution.}

\subsubsection{Gender Analysis of Implicit Mentoring}
The dataset used for analyzing implicit mentoring through the gender lens includes the contributions of 6,342 contributors. Recall, we used Namesor to identify the gender of contributors and only include those individuals for whom the API is able to predict gender with high confidence ($>90\%$), this led us to drop those authors whose gender the API could not reasonably identify.


\input{Table/sec4_gender_overall}
Table \ref{tab:genderoverall} shows the distribution of developers in this dataset with respect to their gender and mentoring activity. A majority of developers---71.48\%---acted as implicit mentors. That is, 4,533 developers were authors of least one PR-comment that was identified as implicit mentoring. This shows that a majority of contributors provide guidance to others. The gender distribution shows that 5.30\% (240) were women and the 94.70\% (4,293) men. 


\boldification{men doing more mentoring than women for overall mentoring approaches, but the effect size and estimated ratio are quite small,  we unpack, we noticed that women are doing more mentoring for bottom-up and top to down...}
\hl{Past research has shown that the conventional view of mentoring is that women tend to do more mentoring than men} \cite{sosik2000role, bianca paper}. 
%Steve found the ref
In our dataset, we see an opposite trend---71.78\% of men provided implicit mentoring as compared to 67.99\% of women. To see if these differences were statistically significant, we performed a two sample Z-test of proportions (see~\ref{sec:method}) between the proportions of PR mentoring provided by men compared to women (see Table ~\ref{tab:gender_overall_Z} (Overall column).

The results for \textit{overall mentoring} show that there is a significant difference ($estimate=0.02, p<0.001$) between men and women, with men mentoring 2.2\% times more as compared to women. Since the estimated ratio of differences is small---0.02, we
calculate effect size using Cohen's d \cite{cohen2013statistical} to investigate the differences between the two groups. An effect size of $d=0.05$ (see Table \ref{tab:gender_overall_Z}, Overall Column) indicates that the differences between the proportion of mentoring provided by men and women are negligible. Note, effect size thresholds of $d=0.2$ is considered small; $d=0.5$ medium, and $d=0.8$  large \cite{cohen2013statistical}.

%Yellow highlight means, AS needs to check if Lit supports this
%I found a paper saying that men are more likely to have formal mentors than women.

\input{Table/sec4_gender_overall_Z}
%One reason for this difference might be because our sample sizes are unequal. Therefore, we used estimated ratio and effect size to further investigate the differences between the groups. The estimated ratio of differences was small --- 0.022 (cf. Table \ref{tab:gender_overall_Z}). 

\vspace{0.3cm}
\begin{mdframed}[roundcorner=10pt]
  \textbf{Observation 3:} Overall, more men than women provide implicit mentoring, but the difference is negligible.
\end{mdframed}
\vspace{0.3cm}


Next, we investigate the different implicit mentoring approaches, such as top-down, peer-to-peer, and bottom-up mentoring. Table \ref{tab:gender_overall_Z}  presents the results of two sample Z-test of proportions and the effect sizes.

When considering \textit{peer mentoring}, more men than women gave implicit mentoring via the PR-comments ($estimate=0.05, p<0.001$). While the differences are significant, the effect size is negligible (Cohen $d=0.11$). 
For \textit{top-down} and \textit{bottom-up} approaches, there are significant differences between the proportion of mentoring given by women and men, but here it is reverse. More women than men provided Top$\rightarrow$Down mentoring ($estimate =-0.10, p<0.001$), showing that women provided 10\% more implicit mentoring than men. The effect size is small (Cohen $d=0.20$). Similarly, more women than men were involved in Bottom$\rightarrow$Up mentoring ($estimate =-0.03, p=0.027$), but with negligible effect size (Cohen $d=0.07$). 
%Since the proportion of women was greater than that of men the $estimate$-score is negative. 
%For bottom-up, the proportion of mentoring for women was 0.028 more than men, and for top-to-down, it was 0.098 more than men. 



\vspace{0.3cm}
\begin{mdframed}[roundcorner=10pt]
  \textbf{Observation 4}: There are significant differences between amounts of implicit mentoring by men and women at the different levels, with men providing more peer-to-peer mentoring and more women providing top-down and bottom-up mentoring. In all cases, however, the differences are negligible or small.
\end{mdframed}
\vspace{0.3cm}

%\noindent\textbf{Observation 4}: There are significant differences between men and women performing mentoring at the different levels, with men doing more peer-to-peer mentoring and women doing more top-down and bottom-up mentoring. In all cases, however, the differences is not large.\leavevmode \\


%In summary, while there are significant differences between men and women performing implicit mentoring, the differences range from negligible to small.

%A possible reason may be because the sample size of peer mentoring is larger than other mentoring approaches, and it may have also affected the overall mentoring proportion test results.  

%\input{Table/sec4_chi2square}

\boldification{Our test indicates that for all identified implicit mentoring approaches, there are gender preferences when people give mentoring}


\begin{figure}[!tbp]
\centering
\includegraphics[width=3.3in]{pic/gender_dist_plot.png}
\caption{Gender distributions of contributors in the projects in our dataset; 22\% projects have no women.}
\label{fig:gender_dist_plot}
\end{figure}

Next we investigate whether there are gender preferences between mentor-mentee pairing in implicit mentoring. Past work has found \textit{homophily}---the tendency for people to seek out or be attracted to those who are similar to themselves---by gender among mentor-mentee pairs~\cite{ADD ME}.
Our results indicate that gender preferences also exist in implicit mentoring. 

Before, analyzing for homophily in implicit mentoring, we first analyze the dataset to ensure whether there are women contributors in the projects for men to mentor. Table~\ref{gender_dist_plot} shows the gender distribution of contributors in the projects in our dataset. Eight projects had no women contributors, so we removed the contributors from these projects---223 contributors (4\% of contributors). 

\input{Table/sec4_homophily_gender_dist}

Table \ref{tab:gender_homophily_dist} (Overall column) presents the number of implicit mentoring comments grouped by the genders of the mentor$\rightarrow$mentee pair. That is, w$\rightarrow$w means a woman mentored another woman and a w$\rightarrow$m means a woman mentored a man. 
classified into the mentoring approach they took (bottom-up, top-to-down, peer mentoring). The largest group of implicit mentoring occurred between men (m$\rightarrow$m, 96.13\% cases), followed by mentoring between women (w$\rightarrow$w, 2.04\% cases). This shows that homophily is present in a majority of cases (98.17\%). 

A ${\chi}^2$ test with Bonferroni correction revealed that every gendered mentor$\rightarrow$mentee pair were statistically different ($p<0.001$). %(${\chi}^2=164884, df=3, p<0.001$).
A two-sample proportionality test (see Table\ref{tab:sec4_homophily_Z}) between homophilic implicit mentoring and cross-gender mentoring found significant differences ($estimate=0.96, p<0.001$) with large effect size (Cohen $d=2.6$).
%
Similar gender preferences in mentor-mentee pairs exist among the different mentoring approaches. Homophilic mentoring surpassed cross-gender mentoring for top-down, peer-to-peer, and bottom-up mentoring with large effect size. See Table\ref{tab:sec4_homophily_Z} for the test results.  

\input{Table/sec4_homophily_Z}

\input{Table/sec4_homophil_cross_gender}
In the small percentage of cases (1.83\%) where cross-gender mentoring occurred, there is evidence that more women than men ``crossed'' gender boundaries when giving mentoring feedback (see Table~\ref{tab:sec4_homophil_cross_gender}, Overall column: $estimate=-0.161, p<0.001$) with medium effect size (Cohen   $d=0.623$). We see similar results for the different mentoring approaches, with more women than men participating in cross-gender mentoring, especially in top-down mentoring which has a large effect size (Cohen $d=1.16$).

\vspace{0.3cm}
\begin{mdframed}[roundcorner=10pt]
\textbf{Observation 5}: Homophily exists in mentor$\rightarrow$mentee pairs for both genders. In the few cases of cross-gender mentoring women tend to cross gender boundaries more often than men.
\end{mdframed}







==> attic/related.tex <==


\deleted{
In the context of research in OSS, several works have identified the lack of mentoring as a challenge for newcomer onboarding~\cite{steinmacher2012recommending, steinmacher2015systematic, fagerholm2014onboarding}. Others have identified the challenges that mentors face in OSS~\cite{balali2018newcomers, balali2020recommending, trinkenreich2020hidden}. Researchers have found that mentoring allowed for a more effective onboarding experience than when newcomers entered a project through a natural, non-deliberate process~\cite{fagerholm2014role, fagerholm2014onboarding}. Google through its formal Google Summer of Code (GSoc) mentorship program aims to facilitate onboarding to OSS~\cite{johnson2010learning}. Several works have investigated the effectiveness of the program~\cite{silva2020google}, the type of contributions made by students~\cite{silva2017long}, and their motivations for joining the program~\cite{silva2020google}.
To the best of our knowledge, no prior work has explored the concept of implicit mentoring in OSS. Our paper fills this gap by investigating how implicit mentoring happens and who are these mentors in the OSS community.}


\boldification{***SE has defined mentoring in these ways.}
%
\deleted{Software Engineering research has investigated mentoring, especially in the context of onboarding activities. Begel and Simon~\cite{begel2008novice} discuss the importance, advantages and challenges of mentoring for novices in the software industry. Kumar and Wallace~\cite{kumar2014communication} investigated communication strategies for mentoring in software development projects, including ``Code As Conversation'' pattern, where participants on the forum ask or answer questions regarding a code snippet that is shared through communication channels. }

==> extra.tex <==
\subsection{Mentoring in OSS}

To get an overview of the current state-of-the-art research in the field of OSS  mentoring, we conduct a literature survey. We focus on the papers from 2012 to 2021 (inclusive) that related to mentorship in top conferences in Software Engineering: IEEE-ICSME, IEEE-RSSE, IEEE-ICGSEW, ACM-FSE, ACM-ESEM, ACM-ICSE, IEEE-ICSME, IEEE-MSR, ACM-SIGCSE, ACM-HCI, and ACM-ICPS.

While conducting the literature survey, we searched for a set of keywords including mentoring in OSS, mentorship in OSS, implicit mentoring in OSS, informal mentoring software engineer etc. We found 23 papers on mentoring in OSS. And Table \ref{tab:literaturesurvey} presents the summary of the literature survey for most recent 10 years. 

\zf{Table may move to appendix later}
\begin{table}[t]
\label{tab:literaturesurvey}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll|l|l|}
\cline{3-4}
                                                                        &                                                                                                                         & \cellcolor[HTML]{FCFF2F}{\color[HTML]{000000} } & Explicit mentoring for newcomers  \\ \cline{3-4} 
                                                                        &                                                                                                                         & \cellcolor[HTML]{FFCE93}                        & Explicit mentoring programs       \\ \cline{3-4} 
                                                                        &                                                                                                                         & \cellcolor[HTML]{9AFF99}                        & Potential implicit mentoring      \\ \hline
\multicolumn{1}{|l|}{\textbf{Index}}                                    & \textbf{Title}                                                                                                          & \textbf{Year}                                   & \textbf{Conference}               \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}1}                         & Recommending Tasks to Newcomers in OSS Projects: How Do   Mentors Handle It?                                            & 2020                                            & ACM-ICPS                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}2}                         & Training the future workforce through task curation in an OSS   ecosystem                                               & 2016                                            & ACM-FSE                           \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}3}                         & Let Me In: Guidelines for the Successful Onboarding of   Newcomers to Open Source Projects                              & 2019                                            & IEEE-journal                      \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}4}                         & Overcoming open source project entry barriers with a portal   for newcomers                                             & 2016                                            & ACM-ICSE                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}5}                         & X marks the task: Helping developers navigate to the right   task                                                       & 2016                                            & IEEE-HCC                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}6}                         & Determining Newcomers Barrier in Software Development: An IT   Industry Based Investigation                             & 2018                                            & ACM-CSCW                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}7}                         & A Simple NLP-Based Approach to Support Onboarding and   Retention in Open Source Communities                            & 2018                                            & IEEE-ICSME                        \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}8}                         & The role of mentoring and project characteristics for   onboarding in open source software projects                     & 2014                                            & ACM-ESEM                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}9}                         & Onboarding in Open Source Software Projects: A Preliminary   Analysis                                                   & 2013                                            & IEEE-ICGSEW                       \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}10}                        & Supporting newcomers in software development projects                                                                   & 2015                                            & IEEE-ICSME                        \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}11}                        & Recommending mentors to software project newcomers                                                                      & 2012                                            & IEEE-RSSE                         \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}12}                        & Onboarding in Open Source Projects                                                                                      & 2014                                            & IEEE-journal                      \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}13}                        & The hard life of open source software project newcomers                                                                 & 2014                                            & ACM-ICSE                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}14}                        & Do Onboarding Programs Work?                                                                                            & 2015                                            & IEEE-MSR                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}15}                        & Who is going to mentor newcomers in open source   projects?                                                             & 2012                                            & ACM-FSE                           \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}16}                        & Communication strategies for mentoring in software development   projects                                               & 2014                                            & ACM-ICSE                          \\ \hline
\rowcolor[HTML]{FFCE93} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFCE93}{\color[HTML]{000000} 17}} & {\color[HTML]{000000} A theory of the engagement in open source projects via summer   of code programs}                 & {\color[HTML]{000000} 2020}                     & {\color[HTML]{000000} ACM-FSE}    \\ \hline
\rowcolor[HTML]{FFCE93} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFCE93}{\color[HTML]{000000} 18}} & {\color[HTML]{000000} How Long and How Much: What to Expect from Summer of Code   Participants?}                        & {\color[HTML]{000000} 2017}                     & {\color[HTML]{000000} IEEE-ICSME} \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 19}} & {\color[HTML]{000000} Hackathons as an Informal Learning Platform}                                                      & {\color[HTML]{000000} 2016}                     & {\color[HTML]{000000} ACM-SIGCSE} \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 20}} & {\color[HTML]{000000} Informal Mentoring of Adolescents about Computing: Relationships, Roles,   Qualities, and Impact} & {\color[HTML]{000000} 2018}                     & {\color[HTML]{000000} ACM-SIGCSE} \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 21}} & {\color[HTML]{000000} GitHub-OSS Fixit: Fixing Bugs at Scale in a Software   Engineering Course}                        & {\color[HTML]{000000} 2021}                     & {\color[HTML]{000000} ACM-ICSE}   \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 22}} & {\color[HTML]{000000} Why is collaboration needed in OSS projects? a case   study of eclipse project}                   & {\color[HTML]{000000} 2013}                     & {\color[HTML]{000000} ACM-FSE}    \\ \hline
\end{tabular}}
\end{table}


\textbf{***Among the state of art we surveyed from top conference in software engineering, only 2 papers address the implicit mentoring plainly and intentionally, and only focus on teenager computing new learners.}
%
Among the state of art we surveyed, that 16 out 22 studies discussed that mentoring for newcomers, and 2 papers addressed official mentoring programs such as summer of code programs \cite{silva2020theory,silva2017long}, and these program still intend to on-board newcomers. We surprised noticed that only 2 papers address the implicit mentoring plainly and intentionally, but limited for certain group of people in  the field of software engineering. 



\subsection{Implicit mentoring in OSS}



\textbf{***Some literature stated that mentoring happens in GitHub when mentors reviews code. Therefore, we noticed that Pull-request and the comments along with may be a channel that implicit mentoring exist, for example, bug-fix, giving suggestions and instructions.}
%
Tan et. al \cite{tan2021github} find that the GitHub, as one of the most popular OSS community, ensure the code quality by using mentors to review codes. And these activities are not limited to explicit mentoring.  
Hayashi et.al \cite{hayashi2013collaboration} address that singly developer in OSS always only has narrow knowledge, collaborations is one of the methods to over difficulties. For example,  if one committer does not have sufficient knowledge of related parts, collaborations must be taken place to verify and commit the bug-fix. This process can be identified as implicit mentoring, since the collaboration can happens randomly, but the the process including addressing issues, giving instructions, etc. 


\textbf{Mentoring has its own set of challenges, one of which is lack of visibility. This lack of visibility can amount to mentors lose their engineering voice. Some research has shown that this is particularly true for women}
%




\zf{Table may move to appendix later}
\begin{table}[t]
\label{tab:literaturesurvey}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll|l|l|}
\cline{3-4}
                                                                        &                                                                                                                         & \cellcolor[HTML]{FCFF2F}{\color[HTML]{000000} } & Explicit mentoring for newcomers  \\ \cline{3-4} 
                                                                        &                                                                                                                         & \cellcolor[HTML]{FFCE93}                        & Explicit mentoring programs       \\ \cline{3-4} 
                                                                        &                                                                                                                         & \cellcolor[HTML]{9AFF99}                        & Potential implicit mentoring      \\ \hline
\multicolumn{1}{|l|}{\textbf{Index}}                                    & \textbf{Title}                                                                                                          & \textbf{Year}                                   & \textbf{Conference}               \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}1}                         & Recommending Tasks to Newcomers in OSS Projects: How Do   Mentors Handle It?                                            & 2020                                            & ACM-ICPS                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}2}                         & Training the future workforce through task curation in an OSS   ecosystem                                               & 2016                                            & ACM-FSE                           \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}3}                         & Let Me In: Guidelines for the Successful Onboarding of   Newcomers to Open Source Projects                              & 2019                                            & IEEE-journal                      \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}4}                         & Overcoming open source project entry barriers with a portal   for newcomers                                             & 2016                                            & ACM-ICSE                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}5}                         & X marks the task: Helping developers navigate to the right   task                                                       & 2016                                            & IEEE-HCC                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}6}                         & Determining Newcomers Barrier in Software Development: An IT   Industry Based Investigation                             & 2018                                            & ACM-CSCW                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}7}                         & A Simple NLP-Based Approach to Support Onboarding and   Retention in Open Source Communities                            & 2018                                            & IEEE-ICSME                        \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}8}                         & The role of mentoring and project characteristics for   onboarding in open source software projects                     & 2014                                            & ACM-ESEM                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}9}                         & Onboarding in Open Source Software Projects: A Preliminary   Analysis                                                   & 2013                                            & IEEE-ICGSEW                       \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}10}                        & Supporting newcomers in software development projects                                                                   & 2015                                            & IEEE-ICSME                        \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}11}                        & Recommending mentors to software project newcomers                                                                      & 2012                                            & IEEE-RSSE                         \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}12}                        & Onboarding in Open Source Projects                                                                                      & 2014                                            & IEEE-journal                      \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}13}                        & The hard life of open source software project newcomers                                                                 & 2014                                            & ACM-ICSE                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}14}                        & Do Onboarding Programs Work?                                                                                            & 2015                                            & IEEE-MSR                          \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}15}                        & Who is going to mentor newcomers in open source   projects?                                                             & 2012                                            & ACM-FSE                           \\ \hline
\rowcolor[HTML]{FCFF2F} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FCFF2F}16}                        & Communication strategies for mentoring in software development   projects                                               & 2014                                            & ACM-ICSE                          \\ \hline
\rowcolor[HTML]{FFCE93} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFCE93}{\color[HTML]{000000} 17}} & {\color[HTML]{000000} A theory of the engagement in open source projects via summer   of code programs}                 & {\color[HTML]{000000} 2020}                     & {\color[HTML]{000000} ACM-FSE}    \\ \hline
\rowcolor[HTML]{FFCE93} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFCE93}{\color[HTML]{000000} 18}} & {\color[HTML]{000000} How Long and How Much: What to Expect from Summer of Code   Participants?}                        & {\color[HTML]{000000} 2017}                     & {\color[HTML]{000000} IEEE-ICSME} \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 19}} & {\color[HTML]{000000} Hackathons as an Informal Learning Platform}                                                      & {\color[HTML]{000000} 2016}                     & {\color[HTML]{000000} ACM-SIGCSE} \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 20}} & {\color[HTML]{000000} Informal Mentoring of Adolescents about Computing: Relationships, Roles,   Qualities, and Impact} & {\color[HTML]{000000} 2018}                     & {\color[HTML]{000000} ACM-SIGCSE} \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 21}} & {\color[HTML]{000000} GitHub-OSS Fixit: Fixing Bugs at Scale in a Software   Engineering Course}                        & {\color[HTML]{000000} 2021}                     & {\color[HTML]{000000} ACM-ICSE}   \\ \hline
\rowcolor[HTML]{9AFF99} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{9AFF99}{\color[HTML]{000000} 22}} & {\color[HTML]{000000} Why is collaboration needed in OSS projects? a case   study of eclipse project}                   & {\color[HTML]{000000} 2013}                     & {\color[HTML]{000000} ACM-FSE}    \\ \hline
\end{tabular}}
\end{table}


Among these papers, most of the papers focus on the importance, challenges, and benefits of the mentoring. We analyze the amount and kinds of the mentoring they investigated. We notice that 14 studies discussed that mentoring for newcomers, and 2 papers discussed the benefits from mentoring programs such as summer of code programs \cite{silva2020theory,silva2017long}, these program still intend to on-board newcomers. We surprised noticed that only 2 papers address the implicit mentoring plainly and intentionally. 


\begin{table}[htb]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll}
\hline
\textbf{Repository}            & \textbf{Language}                     \\ \hline
\rowcolor[HTML]{EFEFEF} 
{\color[HTML]{000000} Archiva} & {\color[HTML]{000000} Java}           \\
Aries                          & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
{\color[HTML]{000000} Beam}    & {\color[HTML]{343434} Java/Python}    \\
Cassandra                      & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Cloudstack                     & Java/Python                           \\
CXF                            & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Geronimo                       & Java                                  \\
Groovy                         & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Hbase                          & Java                                  \\
Hive                           & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Ignite                         & Java/C\#/C++/SQL/JDBC/ODBC            \\
Isis                           & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Jackrabbit                     & Java                                  \\
Jclouds                        & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Jena                           & Java                                  \\
Karaf                          & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Log4j                          & Java                                  \\
Maven                          & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Mesos                          & C++                                   \\
OFBiz                          & Java/Groovy/JavaScript/XML/Freemarker \\
\rowcolor[HTML]{EFEFEF} 
Phoenix                        & Java/SQL                              \\
Qpid                           & Java/C\#/C++/Perl/Python/Ruby         \\
\rowcolor[HTML]{EFEFEF} 
Storm                          & Java                                  \\
Subversion                     & C\#                                   \\
\rowcolor[HTML]{EFEFEF} 
TomEE                          & Java                                  \\
Wicket                         & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Ant                            & Java                                  \\
Camel                          & Java/CML                              \\
\rowcolor[HTML]{EFEFEF} 
FOP                            & Java                                  \\
JMeter                         & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
POI                            & Java                                  \\
Tinkerpop                      & Java                                  \\
\rowcolor[HTML]{EFEFEF} 
Tomcat                         & Java                                  \\
Usergrid                       & Java/JavaScript/PHP/HTML              \\
\rowcolor[HTML]{EFEFEF} 
Hadoop                         & Java                                  \\
Spark                          & Java/Scala/Python/R/SQL/JDBC          \\
\rowcolor[HTML]{EFEFEF} 
Flink                          & Java/Scala                           
\end{tabular}}
\label{tab:apacheprojects}
\end{table}




\begin{table}[tbp]
\centering
\begin{tabular}{lll}
\multicolumn{3}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Top to down}}    \\ \hline
                     & \textbf{Total}      & \textbf{Mentoring}     \\
Male                 & 114,982             & 38,718                 \\
Female               & 1,103               & 486                    \\
\multicolumn{3}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Bottom up}}      \\ \hline
                     & \textbf{Total}      & \textbf{Mentoring}     \\
\textbf{Male}        & 326,59              & 11,133                 \\
\textbf{Female}      & 638                 & 262                    \\
\multicolumn{3}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Peer mentoring}} \\ \hline
                     & \textbf{Total}      & \textbf{Mentoring}     \\
\textbf{Male}        & 164,993             & 58,620                 \\
\textbf{Female}      & 6,549               & 1,995                 
\end{tabular}
\label{tb:gender_pro_count}
\end{table}






%%%%Homophily section

In our study, we find the occurrence of homophily in implicit mentor-mentee pairs for both men and women. There might be multiple reasons behind this, such as unconscious bias against other genders, personal preferences or mentor and mentee's common expectations from the relationship. As McPherson et al.~\cite{} found, connections and friendships are based on social processes and personal preferences and are not randomly made. Therefore, in non-random informal mentorships, it is more likely to find homophily than it is, when assigned formally. Another reason could be the mentee's view of same-gender mentors as being able to empathize with issues specific to their gender~\cite{}. For example, women in OSS might have faced the same barriers which cause them to empathize with the mentee and also know how to best help them. However, we do not know how much of a role these play when it comes to implicit mentoring on OSS projects and further investigation is needed to get a deeper understanding. 

%\textbf{\textit{RQ \#2c: Does implicit mentoring help in knowledge transfer?}}
%Swap et al. describe mentoring as a fundamental knowledge transfer mechanism in companies~\cite{swap2001using}. We posit that as someone gathers more experience in a project, with passing time and continued mentoring, they will need less help. We calculated the correlation between the number of implicit mentoring and experience, measured using the number of days of involvement in a project to check our intuition. Our results did not show a significant correlation of 0.008 ($t$=0.97167, $P$ value=0.331) \zf{old: -0.03 (t=-5.67, p value$<$0.001} between the number of implicit mentoring and experience.

%\vspace{0.3cm}
%\begin{mdframed}[roundcorner=10pt]
%\textbf{Observation 3:} \zf{This sentence is new:} \hl{There is no statistically significant correlation between the experience of contributors and the amount of implicit mentoring they receive.} 

%\zf{old: As contributors gain experience they receive less implicit mentoring} \end{mdframed}
%\vspace{0.3cm}


\textbf{\textit{RQ \#2b: Do complex PRs need more implicit mentoring?}}

Dabbish et al.~\cite{dabbish2012social} showed that visible cues, such as PR-comments made by contributors serve as an important signal of community support (or lack thereof). They found that PR-comments to a commit (or PR) signal that activity is interesting, controversial or worth looking at. It is possible that ``complex'' PRs that address such interesting or controversial changes elicit more PR-comments, including implicit mentoring PR-comments. Recall, we measure the complexity of PRs using two different metrics. Complexity based on the length of the description~\cite{yu2015wait,dabbish2012social} and based on whether a PR was reopened\cite{8719563}.


PRs with more \textit{wordy description} on an average had more implicit mentoring than those with less wordy descriptions. The difference between the two groups was statistically significant (Welch Two Sample t-test, $t$ =25.48, $df$ = 49,161, $P$ value $<$ 0.001). The effect size measured using Cohens d ~\cite{cohen2013statistical} is 0.18 which is nearly small effect (where small size is 0.2). This corroborates the finding that complex pull requests warrant additional attention or guidance.


Next we considered complexity based on whether the PR was \textit{reopened}. 2,606 out of 107,895 PRs had been reopened in our dataset, out of which 1,294 PRs included implicit mentoring. Complex PRs (based on whether it was reopened) on average, had more mentoring than the non-reopened group. The difference in mean was statistically significant (Welch Two Sample t-test, $t$ = 9.31, $df$ = 1,355, $P$ value $<$ 0.001). The effect size measured using Cohens d ~\cite{cohen2013statistical} is 0.36 which is a small to medium effect. Research has found that reopened PRs have lower acceptance rates, more PR-comments, and longer evaluation time, which might mean either these changes might be complex or controversial and thus might need more guidance ~\cite{8762189}.


\vspace{0.3cm}
\begin{mdframed}[roundcorner=10pt]
\textbf{Observation 2:} Complex PRs (reopened and wordy descriptions PRs) include instances of implicit mentoring.\end{mdframed}
\vspace{0.3cm}

==> todo.tex <==
1. experiences days also add years
2. Remove red data


All decimal points/percentages in the paper should be up to 2 decimal points...not 3...so, 23.309% -> 23.31%> Do a full pass on all text/tables, once Iftekhar and I finish reviewing. We dont need to see it....WHY DID YOU REVERT back to 3 decimal places, when you can see the OLD tables are in 2 decimal places, eh? -DONE



I introduced a latex error in method /place where the classifier results are presented --- DONE


Results: It doesnt make sense to say 57% got/gave implicit mentoring. Better to say 23% gave implicit mentoring? I have made these changes. Double check....and if @Iftekhar Ahmed disagrees, revert back --- DONE



Results RQ2a: Check if 27% of PR or PR Comments got implicit mentoring...I think the section maybe confusing one with the other --- DONE


The paper needs a full reading pass. There are tiny (late night/last minute) mistakes. RQ2b: had the "more wordy" was more blah than "more verbose"...similarly....d= blah is between "Median" to large --- DONE



Q: for top-down/bottom-up pair date differences, should we keep it in Days or Convert to months? Since we use 6-month threshold? I mean...what does a difference of 1008.773 days really mean??, but it gets harder to write down the SD?  NOT DONE



4.3.1, needs a detailed pass after all the old/new stuff has been addressed - so its a clean copy. Its a hard section to understand...its so strewn with data. --- DONE


Would Table 6 also not change? I dont see the old Table 6 (summary of implicit mentoring gender) --> Maybe whats in the paper is the new one, since decimal places are in 3 digits --- DONE



@Steve Feng, dude...the Gernder section needs a rewrite...our results (T7)  have flipped when we consider the T->D and the other lenses (W>M in Table 7). BUT, when we consider the overall M>W...How is that possible. Do we need to double check the numbers? Make sure the section is still correct, which might effect Obs. #6 --- DONE


10. In some cases, the old tables are still being referenced in text, so once we clean up the paper, we need to make sure that all cross-references are correct (but do this as a last item) ---WORKING ON

11. For Homophily...I am getting confused with which are large/medium effect size...I think in the old text/table we didnt have large effect size...BUT NOW WE do. So, Text for Table 13 is not incorrect/off....--- DONE


12: Conclusions/FW: is 27% of PRs or PR-comments that had implicit mentoring...this is a confusion being carried on from Results section.....AND again, we dont care about how many geve/recd. Implicit mentoring...but how many gave? This words are likely copied from results...so, if we fix there, we fix here (edited)  --- DONE

13. Bios....nobody cares about our histories...so delete where you got BS etc. Just state your N-1 degree if you want to. I removed that too, since it doesnt matter for me anymore --- DONE


Once these changes are done...I would like to take a look again at Results, especially the Gender Section, since there are quite a few tiny mistakes. --- DONE
